Coarse-Grained Complexity for Dynamic Algorithms

To date, the only way to argue polynomial lower bounds for dynamic algorithms is via fine-grained complexity arguments. These arguments rely on strong assumptions about specific problems such as the Strong Exponential Time Hypothesis (SETH) and the Online Matrix-Vector Multiplication Conjecture (OMv). While they have led to many exciting discoveries, dynamic algorithms still miss out some benefits and lessons from the traditional ``coarse-grained'' approach that relates together classes of problems such as P and NP. In this paper we initiate the study of coarse-grained complexity theory for dynamic algorithms. Below are among questions that this theory can answer. What if dynamic Orthogonal Vector (OV) is easy in the cell-probe model? A research program for proving polynomial unconditional lower bounds for dynamic OV in the cell-probe model is motivated by the fact that many conditional lower bounds can be shown via reductions from the dynamic OV problem. Since the cell-probe model is more powerful than word RAM and has historically allowed smaller upper bounds, it might turn out that dynamic OV is easy in the cell-probe model, making this research direction infeasible. Our theory implies that if this is the case, there will be very interesting algorithmic consequences: If dynamic OV can be maintained in polylogarithmic worst-case update time in the cell-probe model, then so are several important dynamic problems such as $k$-edge connectivity, $(1+\epsilon)$-approximate mincut, $(1+\epsilon)$-approximate matching, planar nearest neighbors, Chan's subset union and 3-vs-4 diameter. The same conclusion can be made when we replace dynamic OV by, e.g., subgraph connectivity, single source reachability, Chan's subset union, and 3-vs-4 diameter. Lower bounds for $k$-edge connectivity via dynamic OV? (see the full abstract in the pdf file).

==> NPcapcoNP.tex <==

\section{$\dNP\cap\dcoNP$}


==> NPhard.tex <==

\section{Some DNP-hard Problems}

\label{sec:reductions}


\paragraph{Preprocessing time.}

For all the dynamic problems we consider, we allow for quasi-polynomial
(in input size) preprocessing time. This is because we have to allow
for this much preprocessing time while defining the complexity class
DP and DNP. {\em Q: Is it necessary to allow for quasi-polynomial
preprocessing time?}


\paragraph{The ``All White\textquotedbl{} problem.}

Recall the {\em all-white} problem defined in Section~\ref{sec:DP:DNP}.
Theorem~\ref{th:allwhite:DNPcomplete} states that this problem is
DNP complete. We will now give reductions from this problem to various
other problems, which will show that the latter problems are all DNP
hard.


\paragraph{Reduction to dynamic max-flow on a directed capacitated graph.}

Take the input graph $G=(L\cup R,E)$ for the All White problem. Orient
every edge in $E$ from $L$ to $R$ and assign a capacity of $1$.
Create a sink node $t$. For every black node $r\in R$, add a directed
edge $(r,t)$ with capacity $|L|$. Create a source node $s$ and
add a directed edge $(s,l)$ with capacity $1$, for every node $l\in L$.
Now, note that the value of maximum $s-t$ flow in this graph is $|L|$
iff no node $l\in L$ has an all white neighborhood. When we are asked
to change the color of a node $r\in R$ from black to white (resp.
white to black), we simply delete (resp. insert) the edge $(r,t)$
with capacity $|L|$.


\paragraph{Reduction to dynamic subgraph connectivity.}

In the dynamic subgraph connectivity problem, we are given a fixed
input graph. The update consists of turning a node in this graph ``on\textquotedbl{}
or ``off\textquotedbl{}. We have to maintain if the subgraph induced
by the ``on\textquotedbl{} nodes is connected or not. For the reduction,
take the input graph $G=(L\cup R,E)$ for the All White problem. Add
a node $s$ and insert an (undirected) edge $(s,r)$ for every node
$r\in R$. The nodes in $L$ are turned ``on\textquotedbl{}. The
node $s$ is turned ``on\textquotedbl{}. And every black node in
$R$ is turned ``on\textquotedbl{}. Finally, every white node in
$R$ is turned ``off\textquotedbl{}. Note that the subgraph induced
by the ``on\textquotedbl{} nodes is connected iff in the All White
instance there is no node $l\in L$ with an All White neighborhood.


\paragraph{Reduction to dynamic $(4/3-\epsilon)$-approximate diameter.}

Take the input graph $G=(L\cup R,E)$ for the All White problem. Add
a node $s$, and add an (undirected) edge $(s,l)$ for every node
$l\in L$. Add a node $t$, and add an (undirected) edge $(r,t)$
for every black node $r\in R$. Note that the diameter of this new
graph is $3$ if every node $l\in L$ has a black neighbor, and the
diameter is $\geq4$ if there is some node $l\in L$ with an All White
neighborhood.


\paragraph{Reduction to dynamic $S-T$ reach.}

In the dynamic $S-T$ reach problem, we are given a dynamic directed
graph undergoing a sequence of edge insertions/deletions, and two
fixed subsets of nodes $S$ and $T$. The goal is to maintain if every
node in $T$ is reachable from every node in $S$. For the reduction,
take the input graph $G=(L\cup R,E)$ for the All White problem. Orient
every edge in $E$ from $R$ to $L$. Add a node $s$, and add a directed
edge $(s,r)$ for every black node $r\in R$. Set $S=\{s\}$ and $T=L$.
Note that every node in $T$ is reachable from every node in $S$
iff every node $l\in L$ has at least one black neighbor.


\paragraph{Reduction to dynamic count-reach.}

In the dynamic count-reach problem, we are given a dynamic directed
graph undergoing a sequence of edge insertions/deletions, and a fixed
source node $s$. We have to maintain the number of nodes running
reachable from $s$. For the reduction, take the input graph $G=(L\cup R,E)$
for the All White problem. Orient every edge in $E$ from $R$ to
$L$. Add a node $s$, and add a directed edge $(s,r)$ for every
black node $r\in R$. Note that the number of nodes reachable from
$s$ is equal to $|L|+$ no of black nodes in $R$ iff every node
$l\in L$ has at least one black neighbor.


\paragraph{Reduction to dynamic count-SCC.}

In the dynamic count-SCC problem, we are given a dynamic directed
graph undergoing a sequence of edge insertions/deletions. We have
to maintain the number of strongly connected components (SCCs) in
this dynamic graph. For the reduction, take the input graph $G=(L\cup R,E)$
for the All White problem. Orient every edge in $E$ from $R$ to
$L$. Add a new node $s$. Add a directed edge $(l,s)$ for every
node $l\in L$. Add a directed edge $(s,r)$ and a directed edge $(r,s)$
for every black node $r\in R$. Now, note that the number of SCCs
in the resulting graph is equal to $1+$ the number of white nodes
iff every node $l\in L$ has a black neighbor.


\paragraph{Reduction from SETH to dynamic all white.}

Take any SETH instance with $n$ variables and $O(n)$ clauses. Let
$C$ denote the set of all clauses. Partition the variables into two
equal sized subsets: $X_{1}$ and $X_{2}$ -- each of size $n/2$.
Let $U_{1}$ (resp. $U_{2}$) denote the set of all $2^{n/2}$ partial
assignments to the variables in $X_{1}$ (resp. $X_{2}$). Create
a node for every partial assignment in $U_{1}$, and a node for every
clause in $C$. For all $u_{1}\in U_{1}$ and $c\in C$, create an
(undirected) edge $(u_{1},c)$ iff $u_{1}$ {\em does not} satisfy
the clause $c$. Let $N=|U_{1}|$. Then note that $|C|=\Theta(\log n)$.
Hence, the newly created graph has $\Theta(N)$ nodes and $O(N\log N)$
edges. Now, we iterate over $|U_{2}|$ {\em phases}. In each phase,
we take a partial assignment $u_{2}\in U_{2}$, and color every clause
$c\in C$ satisfied by $u_{2}$ as white and every clause $c\in C$
unsatisfied by $u_{2}$ as black. We then ask our dynamic algorithm
for the all white problem if there is a node $u_{1}\in U$ with an
all-white neighborhood. If the answer is yes, then we know that $(u_{1},u_{2})$
will give us a satisfying assignment. If the answer is no, then we
know that the partial assignment $u_{2}$ cannot be part of any satisfying
assignment. In each phase, we have to change the color of $O(\log N)$
nodes, and we have $O(N)$ phases. Thus, after $O(N\log N)$ updates
for the all-white problem, we will be able to figure out the answer
to the satisfiability problem. Hence, if the dynamic algorithm for
the all-white problem has $O(\text{poly}\log N)$ update time, then
we can solve the satisfiability problem in $O(N\cdot\text{poly}\log N)=O(2^{n/2}\cdot n)$
time, which will contradict SETH.


==> OLD_intro.tex <==


\section{OLD intro}











\subsection{Formalization: Bit-Probe Model, $\dP$ and $\dNP$ (Details in \Cref{part:formalization})} As our main result concerns the bit-probe model, we now define relevant complexity classes in this model. 
Recall that the bit-probe model is similar to the RAM model, but the time complexity is measured by the number of memory reads and writes (``probes''); other operations are free. (See \Cref{sec:model} for details.) 
Also recall that for the purpose of arguing
about lower bounds, it is sufficient to do so in this model, since a lower bound in this model implies a lower bound in the RAM model.
Finally, note that all classes defined on the bit-probe model below ($\dP$, $\dNP$ and $\drankNP$) do not change when defined on the cell-probe model with word size $O(\log n)$. 

We need to first discuss what an analogue of P should mean for dynamic algorithms. 
We believe that a natural choice is to consider when each update can be handled in polynomial time in the {\em update size}. Here, the update size refers to the maximum size of the updates the algorithm can possibly get; for example, for dynamic graph problems where each update is an edge insertion and deletion, the update size is $O(\log n)$, where $n$ is the number of nodes which is usually fixed throughout the updates. Just like previous works in the bit- or cell-probe model (e.g. \cite{Miltersen99cellprobe}), we do not restrict the preprocessing time (beyond the fact that the small update time implies that the space used cannot be too large; see \Cref{sec:class} for further discussions). We let $\dPprb$ (or simply $\dP$ when it is clear from the context) denote the class of problems that admit this type of algorithms in the bit-probe model; see \Cref{def:P} for the detailed definition of this class.



For many dynamic problems, being in $\dP$ means being efficiently solvable in the bit-probe model. For example, known algorithms for priority queues, disjoint-set data structures, dynamic range searching and link/cut trees imply that the corresponding problems are in $\dP$, and the question ``Does a dynamic graph problem $X$ under edge updates admit a polylogarithmic-update-time algorithm in the bit-probe model?'' can be rephrased as ``Is $X\in \dP$?''. See \Cref{table:P} a list of some problems in $\dP$. 
Note that it can be assumed that the update size is at least logarithmic of the input size, since it needs to point to update locations in the input. 

\paragraph{$\dNP$:}
We now discuss one natural analogue of the class NP for dynamic problems considered in this paper, denoted by $\dNPprb$ (or $\dNP$ when the context is clear). We only discuss this class informally here; see \Cref{def:NP} for its detailed definition.
Similar to NP in the static setting, $\dNP$ is informally the set of all decision dynamic problems such that the ``yes'' instances have efficiently verifiable proofs, with the difference being that the proof itself is a {\em dynamic object}. Before getting deeper into the definition, let us first consider an example. 


\begin{example}\label{ex:connectivity in NP}
	Consider the dynamic graph connectivity problem, where we want a polylogarithmic-update-time algorithm to output ``yes'' when the dynamic $n$-node graph $G$ (undergoing edge insertions/deletions) is connected. Additionally, there is a {\em prover} that provides some additional small information to the algorithm during the updates, but the prover cannot be trusted. Is there a protocol so that (i) if the prover follows the protocol, then the algorithm outputs ``yes'' every time $G$ is connected, and (ii) no matter what the prover does, the algorithm never outputs ``yes'' when $G$ is not connected? 
	
	If the answer to this question is yes, then we say that the dynamic graph connectivity problem is in $\dNP$.
	This is indeed the case. One possible protocol is to compute a spanning forest $T$ of the input graph during the preprocessing, then ask the prover to {\em keep updating $T$ so that it remains a spanning forest}. It is not hard to see that at most one edge insertion is needed after each edge update in $G$\footnote{\label{foot:intro:no_delete_connectivity}If an edge is $T$ is deleted from $G$, we can delete it ourselves. There is no need for the prover to tell us.}.
	 %
	If the prover follows this protocol, our algorithm can correctly outputs ``yes'' whenever $T$ has $n-1$ edges (and thus should be a spanning tree), and ``no'' otherwise. Using the fact that we can detect in polylogarithmic time if the prover tries to insert an edge that causes a cycle in $T$ (using, e.g., link/cut tree or top tree data structures \cite{SleatorT81,AlstrupHLT05}), it is not hard to see that we can avoid saying ``yes'' when the graph is not connected no matter what the prover does.\footnote{In more details: Two ways that the prover may deviate from the protocol are (i) inserting an edge to $T$ that causes a cycle in an attempt to fool us that $T$ is a spanning tree, or (ii) not updating $T$ when an edge can actually be inserted, making $T$ not a spanning forest. The first case can be detected, and we can keep outputting ``no'' afterwards. The second case will only cause us to answer ``no'' when the graph is connected, but not vice versa.}
\end{example}

The example above can be generalized to the following informal definition of $\dNP$: we say that a decision dynamic problem $X$ is in $\dNP$ if there is an efficient dynamic algorithm $V$, called ``verifier'', and a protocol between a prover and verifier such that (i) if the prover follows the protocol, then the verifier outputs ``yes'' at all yes-instances of $X$, and (ii) no matter what the prover does, the verifier never outputs ``yes'' at no-instances.
It might be a fun exercise for readers to show that the decision/gap versions of the following problems are in $\dNP$: $(1+\epsilon)$-approximate matching, planar nearest neighbor, and dynamic 3SUM; see \Cref{table:BPP-NP} for their definitions and for other problems in $\dNP$ that are not known to be in $\dP$, and see \Cref{sec:app:classification} for proofs that they are in $\dNP$. 


To this end, note that clearly $\dP\subseteq \dNP$. Given that $\dNP$ contains a large number of natural problems, many of which are not known to be in $\dP$, proving that $\dP=\dNP$ will be a major breakthrough\footnote{This will imply significant improvements over, e.g., cell-probe upper bounds for the uMv problem in \cite{LarsenW17} and communication complexity of the disjointness problem by \cite{ChattopadhyayEEP12} in the 3-party model of \cite{Patrascu10}. 
Moreover, this also implies that the hope to extend the cell-probe lower bounds for the multiphase problem and the uMv problem in restricted settings by \cite{CliffordGL15} and  \cite{ChakrabortyKL17} to the unrestricted one is impossible.}, if possible at all.




\subsection{The Class $\drankNP$ and $\drankNP$-Completeness (Details in \Cref{part:completeness})} Our main result is the completeness proof for a class between $\dP$ and $\dNP$ called $\drankNP$. This seems to be a very big class as it contains all natural we know to be in $\dNP$ so far.
Its definition is similar to $\dNP$, but require the protocol to be defined by some {\em validity and rank functions} over on all possible proofs. 
Let us again start with an example.

\begin{example}
	\label{ex:connectivity in rankNP} Consider the protocol in \Cref{ex:connectivity in NP}. 
	It can be interpreted as being defined by the following validity and rank functions. 
	Recall that possible proofs that the prover can send to the verifier after each update is an edge update to $T$; i.e. the proof after each update to $G$ is a message telling the verifier to either insert an edge to $T$ or do nothing.\footnote{Again, the verifier can delete an edge from $T$ him/herself; see \Cref{foot:intro:no_delete_connectivity}.}
	 %
	 We say that a proof is {\em valid} if it keeps $T$ as a (not necessarily spanning) forest. In other words, invalid proofs are edge insertions that cause a cycle in $T$. An invalid proof can be detected in polylogarithmic time by the verifier (using, e.g. link/cut or top-trees). We {\em rank} the proofs by putting ``do nothing'' last (other proofs can be ordered arbitrarily). 
	Now we say that the prover follows the protocol if s/he sends a valid proof that is ranked first; in other words, we ask the prover to ``insert an edge to $T$ if possible and otherwise do nothing'' after each update. It it not hard to see that if the prover follows the protocol then $T$ is always a spanning forest. If s/he does not, either the verifier can detect an invalid proof and always output ``no'' afterwards, or $T$ is not a spanning forest. In either case, the verifier will not output ``yes'' when $G$ is not connected.
	\qed
\end{example}

The example above can be generalized to the following informal definition of $\drankNP$ (see \Cref{def:rankNP} for the detailed definition):
We say that a decision dynamic problem $X$ is in $\drankNP$ if it admits the following type of protocol. 
At any point in time, any proof sent from the prover to the verifier will be marked by the verifier as {\em valid} and {\em invalid}. There is a {\em rank} function that defines a total order among all possible proofs that can be sent from the prover (e.g. rank among the updates to $T$ in \Cref{ex:connectivity in rankNP}). This rank function must be {\em global} in the sense that it does not change over time (in \Cref{ex:connectivity in rankNP} inserting an edge is always preferred over doing nothing). We say that the prover {\em follows} the protocol defined by this validity and rank functions if s/he sends to the verifier the {\em first valid proof}. We want the same constraints as for $\dNP$ to hold with this type of protocol; i.e.  (i) if the prover follows the protocol, then the verifier outputs ``yes'' at all yes-instances of $X$, and (ii) no matter what the prover does, the verifier never outputs ``yes'' at no-instances. 
Examples of problems in $\drankNP$ (which are all we know to be in $\dNP$) are in \Cref{table:BPP-NP}.





\paragraph{Our Main Result: $\drankNP$-Completeness/Hardness.}
Our main result is the $\drankNP$-completeness of the following problem called {\em dynamic narrow
DNF evaluation problem} (in short, $\dDNF$; details in \Cref{def:range DNF}): Initially, we are given to preprocess (i) an $m$-clause $n$-variables DNF formula\footnote{Recall that a DNF formula is in the form $C_{1}\vee\dots\vee C_{m}$, where each ``clause'' $C_i$ is a conjunction (AND) of literals.} where each clause contains $O(\polylog(m))$ literals, and (ii) (boolean) values of variables. Each update is a change of the value of one variable. After each update, we have to answer whether the DNF formula is true or false. 


It is not hard to see that this problem is in $\drankNP$: the proof is simply a pointer to the clause that is true. 
A naive algorithm for this problem is to keep track of the values of all clauses, but this may take a long update time if the updated variable is in many clauses. If this problem is in $\dP$, then it will have a much faster algorithm, that with polylogarithmic update time. Our proof that it is $\drankNP$-complete implies that this might be unlikely:



\begin{thm}(Details in \Cref{sec:DNF})
	If $\dDNF\in \dP$, then $\dP=\drankNP$.
\end{thm}

To formally state what $\drankNP$-completeness really means, we need more definitions (e.g. the notion of $\dP$-reduction (cf. \Cref{def:P-reduction})). We defer this to later sections. 


\begin{cor}
	All problems in \ref{table:NP hard} (e.g.  approximate diameter, subgraph connectivity and maximum flow) 
	are $\drankNP$-hard. In other words, unless $\dP=\drankNP$, these problems are not in $\dP$. 
\end{cor}

Note that lower bounds (in RAM) for problems in \Cref{table:NP hard} were already known by assuming SETH \cite{AbboudW14}. 
Our $\drankNP$-hardness results suggest that these problems might not admit efficient dynamic algorithms even in the bit-probe model. 
The proof of \Cref{table:NP hard} simply follows from observing that $\dDNF$ is equivalent to a dynamic version of the Orthogonal Vector (OV) problem, which we call $\dOV$ (cf. \Cref{def:OV}), and that all reductions in \cite{AbboudW14} are indeed reductions from $\dOV$ or problems reducible from $\dOV$.




\subsection{Back to RAM (Details in \Cref{part:RAM})}

One can define complexity classes similar to $\dPprb$, $\dNPprb$, and $\drankNPprb$, in the RAM model. We let  $\dPram$, $\dNPram$, and $\drankNPram$ denote such classes. Can we say anything about these classes and $\dDNF$ in the RAM model? 

First we show that some known conjectures imply some separations between these classes.
Assuming %
either SETH \cite{ImpagliazzoP01} and OMv \cite{OMV}, we show lower bounds of update time of algorithms for $\dDNF$ which imply that 
$\dPram \neq \dNPram$. By assuming the nondeterministic version of SETH \cite{CarmosinoGIMPS16}, we can also show that $\dcoNPram \neq \dNPram$.



Next, we show that $\dDNF$ is complete in a complexity class similar to $\drankNPram$ in a {\em relaxed} RAM model, where the space is allowed to be exponential in the update size.
In particular, let $\relaxed\dPram$ and $\relaxed\drankNPram$ be classes in the relaxed RAM model similar to  $\dPram$  and $\drankNPram$. Then, we can show that if $\dDNF$ is in $\relaxed\dPram$, then 
$\relaxed\dPram=\relaxed\drankNPram$.  Note that if $\relaxed\dPram=\relaxed\drankNPram$, then there are polylogarithmic-update-time algorithms for those $\drankNPprb$-hard problems in \Cref{table:NP hard} that use quasi-polynomial space, a rather surprising result.


\subsection{Organization}

Getting definitions right are an important part of proving completeness results. This is done in \Cref{part:formalization}. In particular, we formally define the notion of dynamic problems and dynamic algorithms on the bit-probe model in \Cref{sec:model}, basic complexity classes ($\dP$ and $\dNP$) and examples of problems in these classes in \Cref{sec:class}, and the notions of reductions, hardness and completeness in \Cref{sec:reduction}.

\Cref{part:completeness} is devoted to proving our main result, the $\drankNP$-completeness and hardness in the bit-probe model. We define the complexity class $\drankNP$ in \Cref{sec:rankNP}. \Cref{sec:DT} is devoted to proving the $\drankNP$-hardness of an intermediate problem called {\em First Shallow Decision Tree}. Then in \Cref{sec:DNF} we prove $\drankNP$-completeness of $\dDNF$ and other equivalent problems. As stated earlier, this immediately implies that many well-known dynamic problems are $\drankNP$-hard. 

We discuss the RAM model in \Cref{part:RAM}. \Cref{sec:DNF conjecture} discusses lower bounds $\dDNF$ under various known assumptions (OMv, SETH, NSETH). In \Cref{sec:RAM complete}, we show that $\dDNF$ is complete in the $\drankNP$ class in a relaxed RAM model. 

\subsection{Related works}
There are several previous attempts to classify dynamic problems.
First, there is a line of works called ``dynamic complexity theory''
(see e.g. \cite{DattaKMSZ15,WeberS05,SchwentickZ16}) where the general
question asks whether a dynamic problem is in the class called $\mbox{DynFO}$.
Roughly speaking, a problem is in $\mbox{DynFO}$ if it admits a dynamic
algorithm expressible by a first-order logic. This means, in particular, that given
an update, such algorithm runs in $O(1)$ parallel time, but might
take arbitrary $\mbox{poly}(n)$ works when the input size is $n$.
A notion of reduction is defined and complete problems of $\mbox{DynFO}$
and related classes are proven in \cite{HesseI02,WeberS05}.
However, as the total work of algorithms from this field can be large
(or even larger than computing from scratch using sequential algorithms), they do
not give fast dynamic algorithms in our sequential setting. 
Therefore, this setting is somewhat irrelevant to our setting.

Second, a problem called the \emph{circuit evaluation} problem has been shown to be
complete in the following sense. First, it is in $\mathsf{P}$ (the
class of static problems). Second, if the dynamic version of circuit
evaluation problem, which is defined as $\dDNF$ where a DNF-formula
is replaced with an arbitrary circuit, admits a dynamic algorithm
with polylogarithmic update time, then for any static problem $L\in\mathsf{P}$,
a dynamic version of $L$ also admits a dynamic algorithm with polylogarithmic
update time. This idea is first sketched informally since 1987 by
Reif \cite{Reif87}. Miltersen et al. \cite{MiltersenSVT94} then
formalized this idea and showed that other $\mathsf{P}$-complete
problems listed in \cite{miyano1990list,greenlaw1991compendium} also
are complete in the above sense\footnote{But they also show that this is not true for all $\mathsf{P}$-complete
	problems.}. The drawback about this completeness result is that the dynamic
circuit evaluation problem is extremely difficult. 
Similar to the case for static problems that reductions from $\mathsf{EXP}$-complete problems to problems in $\mathsf{NP}$ are unlikely, 
reductions from the dynamic circuit evaluation problem to other natural dynamic problems studied in the field seem unlikely. 
Hence, this does not give a framework for
proving hardness for other dynamic problems. 

Our result can be viewed as a much more fine-grained completeness
result than the above. As we show that a very special case of the
dynamic circuit evaluation problem which is $\dDNF$ is already a
complete problem. An important point is that $\dDNF$ is simple enough
that reductions to other natural dynamic problems are possible. 

Last, Ramalingam and Reps \cite{RamalingamR96} classify dynamic problems
according to some measure\footnote{They measure the complexity dynamic algorithms by comparing the update
	time with the size of \emph{change in input and output }instead of
	the size of input itself.}, but did not give any reduction and completeness result. Yin \cite{Yin10}
considers the nondeterministic cell-probe model and give some unconditional
lower bounds, but does not give any completeness result as well.

==> RAM.tex <==

\section{Complexity of the $\protect\dAW$ Problem in Uniform Models}
\begin{itemize}
\item Show reduction 

\begin{itemize}
\item Proof: OMv = allwhite (degree 2) 
\end{itemize}
\item Corollary 

\begin{itemize}
\item OMv as a single conjecture for all dynamic problems 
\item If Allwhite in NP \textbackslash{}cap coNP (RAM), then NSETH is false. 
\item If Allwhite in BPP (RAM), then SETH and OMv are false. \end{itemize}
\end{itemize}



==> RAM_DNF.tex <==

\section{Hardness of $\protect\dDNF$ in RAM}

\label{sec:DNF conjecture}

We now consider the standard RAM model where each cell contains logarithmically
many bits. In this model, we can also define natural classes of dynamic
problems. For each complexity class in the bit-probe model defined
in \ref{sec:class}, we can define an analogous class in the RAM model
with two differences. 

First, algorithms in the RAM model are uniform (i.e. the same algorithm
handles all instances of any size), while in the bit-probe model we
have algorithm-families. Second, we believe that it is natural to
allow only $\poly(n)$ preprocessing time, given an initial instance
of size $n$ in the preprocessing step. This is in contrast with in
the bit-probe model, where algorithms in the preprocessing step are
determined by an arbitrary preprocessing function $\init$ which corresponds
to unlimited time. 

Given these two differences, it is clear how to give precise definitions
and, to avoid too much repetition, we show them in \ref{sub:def class RAM }.
To distinguish classes in the RAM and bit-probe models, we now write $\dPram$ and $\dPprb$ to denote the
class $\dP$ in the RAM model and the bit-probe model respectively.
We do similarly for other classes (e.g. $\dNPram$ and $\dNPprb$). 

In this section, we give a quick observation that, by assuming some
conjectures, lower bounds for the update time of algorithms for $\dDNF$
follows easily. Our hardness results are based on three conjectures:
the strong exponential time hypothesis (SETH) \cite{ImpagliazzoP01}
and its nondeterministic variant (NSETH) \cite{CarmosinoGIMPS16},
and the online matrix-vector multiplication conjecture (OMv) problem
\cite{OMV}. 
\begin{thm}
\label{thm:DNF hardness}Let $\A$ be a dynamic algorithm for $\dDNF$
such that, given an $m$-clause formula $\A$ takes $\poly(m)$ preprocessing
time. For any constant $\epsilon>0$, the followings hold.
\begin{enumerate}
\item \label{enu:OMv hardness} Assuming the OMv conjecture, the update time of $\A$ cannot be $O(m^{0.5-\epsilon})$.

\item \label{enu:SETH hardness} Assuming SETH, the update time of $\A$ cannot be $O(m^{1-\epsilon})$.

\item \label{enu:NSETH hardness} Assuming NSETH, the update time of $\A$ cannot be $O(m^{1-\epsilon})$
even if $\A$ is \emph{``nondeterministic''} in the sense that will be made precise in \ref{lem:NSETH hardness}.
\end{enumerate}
\end{thm}



As $\dDNF\in\dNPram$, we obtain the following
class separations:
\begin{cor}
The following holds:
\begin{enumerate}
\item $\dNPram\not\subseteq\dPram$ assuming the OMv conjecture or SETH.
\item $\dNPram\not\subseteq\dcoNPram$ assuming NSETH. 
\end{enumerate}
\end{cor}
The rest of this section is for proving \ref{thm:DNF hardness}. The
reductions are quite standard.


\subsection{OMv-hardness of $\protect\dDNF$ }

\label{sub:DNF:OMvhard}

Here, we show the hardness of $\dDNF$ based on the OMv conjecture.
It is shown in \cite{OMV} that the following variant of independent
set query problem is hard:
\begin{prop}
[Theroem 2.12 of \cite{OMV}]\label{prop:OMV indep}Suppose that the OMv
conjecture holds. For any constant $\epsilon>0$, there is no algorithm
$\A$ (in the RAM model) that, for any $n$, can do the following:
\begin{enumerate}
\item Given an $n$-node (ordinary) graph $G=(V,E)$, then $\A$ preprocesses
in $\poly(n)$.
\item Then, given an online sequence of sets $S_{1},\dots,S_{n}\subseteq V$,
decide if $S_{i}$ is an independent set before $S_{i+1}$ arrives,
using total time $O(n^{3-\epsilon})$.
\end{enumerate}
\end{prop}
Given this, it is immediate how to lower bound the update time of
any $\dDNF$ algorithm:
\begin{lem}
\label{thm:OMv hard}Assuming the OMv conjecture, for any constant
$\epsilon>0$, there is no algorithm for the $\dDNF$ problem on an
$m$-clause formula with $\poly(m)$ preprocessing time and $O(m^{0.5-\epsilon})$
update time. \end{lem}
\begin{proof}
Suppose there is such an algorithm. By \ref{prop:DNF equiv}, there
is an algorithm $\A$ for $\dIndep$ with $\poly(m)$ preprocessing
time and $O(m^{0.5-\epsilon})$ update time. Then, we can solve the
problem from \ref{prop:OMV indep} in time $O(n^{3-\epsilon})$ as
follows. Given an $n$-node $m$-edge $G$, then $\A$ preprocesses
$G$ in $\poly(m)=\poly(n)$. Note that $m\le n^{2}$ as $G$ is an
ordinary graph. Then there are $n$ phases. In the phase $i$, we
update the set $S$ from the definition of $\dIndep$ so that $S=S_{i}$.
At this point, $\A$ returns yes iff $S_{i}$ is independent in $G$.
As there are $n$ updates in each phase, the total time over all $n$
phases is $n\times n\times O(m^{0.5-\epsilon})=O(n^{3-2\epsilon})$.
This contradicts the OMv conjecture.
\end{proof}
This implies \ref{enu:OMv hardness} of \ref{thm:DNF hardness}.


\subsection{SETH-hardness of $\protect\dDNF$ }

\label{sub:DNF:OVhard}

The following variant of the \emph{orthogonal vector problem} \cite{Williams05}
is shown to be hard in the following sense:
\begin{prop}
[\cite{Williams05,AbboudW14}]\label{prop:SETH OV}Suppose SETH holds.
For any constant $\epsilon>0$, there is no algorithm $\A$ (in the
RAM model) such that, for any $n$, when $\A$ is given $U\in\{0,1\}^{n^{c}\times d}$
and $V\in\{0,1\}^{d\times n}$ where $d=\omega(\log n)$ and $c$
is some constant, then $\A$ can decide whether $U\times V$ contains
a zero entry in time $O(n^{c+1-\epsilon})$.
\end{prop}
In other word, let $u_{i}$ and $v_{i}$ be the $i$-th row of $U$
and the $i$-th column of $V$, respectively. We would like to check
if there are $i\in[n^{c}]$ and $j\in[n]$ where $u_{i}\cdot v_{j}=0$,
i.e. $u_{i}$ and $v_{j}$ are orthogonal. Given \ref{prop:SETH OV},
it is trivial to show the hardness of $\dDNF$ in the RAM model. A
similar proof is shown many times in previous literature (e.g. \cite{AbboudW14}).
We include it for completeness. 
\begin{thm}
\label{thm:SETH hard}Assuming SETH, for any constant $\epsilon>0$,
there is no algorithm for the $\dDNF$ problem on an $m$-clause formula
with $\poly(m)$ preprocessing time and $O(m^{1-\epsilon})$ update
time. \end{thm}
\begin{proof}
Suppose there is such an algorithm. By \ref{prop:DNF equiv}, there
is an algorithm $\A$ for $\dOV$ with preprocessing time $O(m^{c})$
for some constant $c$ and $O(m^{1-\epsilon})$ update time. Given
$U\in\{0,1\}^{m^{c}\times n}$ and $V\in\{0,1\}^{n\times m}$, we
use can $\A$ to decide if $U\times V$ contains a zero entry in time
$\tilde{O}(m^{c+1-\epsilon})$ when $n=\polylog(m)$. This contradicts
SETH.

The reduction is straightforward. We create an instance $(V',u')$
for $\dOV$ as follows. Set $V'=V$. As $n=\polylog(m)$, each column
$v_{i}$ is sparse i.e. $nnz(v_{i})=\polylog(m)$. So $V'$ satisfies
the condition in \ref{def:OV}. Then there are $m^{c}$ phases. In
the phase $i$, we update $u'$ so that $u'=u_{i}$ and check if there
is a column $v$ in $V$ where $u'^{T}v=0$. If the answer is yes
in any phase, then there is orthogonal vectors $u\in U$ and $v\in V$.
As there are $n$ updates in each phase, the total time over all $m^{c}$
phases is $n\times m^{c}\times O(m^{1-\epsilon})=\tilde{O}(m^{c+1-\epsilon})$.
\end{proof}
This implies \ref{enu:SETH hardness} of \ref{thm:DNF hardness}.


\subsection{NSETH-hardness for $\protect\dDNF$}

\label{sub:DNF:NSETHhard}

The nondeterministic strong exponential time hypothesis (NSETH) is
a nondeterministic variant of SETH defined by Carmosino et al. \cite{CarmosinoGIMPS16}.
By the same reduction in \cite{AbboudW14}, the following holds similarly
to \ref{prop:SETH OV}:
\begin{prop}
\label{prop:NSETH OV}Suppose NSETH holds. For any constant $\epsilon>0$,
there is no \emph{nondeterministic} algorithm $\A$ (in the RAM model)
such that, for any $n$, when $\A$ is given $U\in\{0,1\}^{n^{c}\times d}$
and $V\in\{0,1\}^{d\times n}$ where $d=\omega(\log n)$ and $c$
is some constant, then $\A$ can decide whether $U\times V$ contains
a zero entry in time $O(n^{c+1-\epsilon})$.
\end{prop}
Here, when we say that a nondeterministic algorithm $\A$ can decide
whether decide whether $U\times V$ contains a zero entry, we mean
there for any $U$ and $V$, there is a proof $\pi_{U,V}$ additionally
given to $\A$ so that $\A$ can verify if $U\times V$ contains a
zero entry \emph{or }not ($\A$ must be able to verify in both cases). 

Given \ref{prop:NSETH OV}, we obtain the following hardness for $\dDNF$
problem by the same proof as in \ref{thm:SETH hard} (so we omit the
proof in this version):
\begin{lem}
\label{lem:NSETH hardness}Assuming NSETH, for any constant $\epsilon>0$,
there is no nondeterministic algorithm for the $\dDNF$ problem on
an $m$-clause formula with $\poly(m)$ preprocessing time and $O(m^{1-\epsilon})$
update time. More precisely, there is no algorithm $\A$ such that
following holds:
\begin{enumerate}
\item In preprocessing step, given an instance $(F,\phi)$ of $\dDNF$ where
$F$ has $m$-clause. Then $\A$ takes $\poly(m)$ time.
\item In each update step $t\ge1$, given an update to $\phi$ together
with a proof-update $\pi_{t}\in\{0,1\}^{O(m^{1-\epsilon})}$. Then
$\A$ takes $O(m^{1-\epsilon})$ time. 
\item For any sequence of updates to $\phi$, there is a sequence of proof-updates,
which is inductively constructed, so that $\A$ can correctly decide
if $F(\phi)=1$ in each step.
\end{enumerate}
\end{lem}
This implies \ref{enu:NSETH hardness} of \ref{thm:DNF hardness}.


==> abstract.tex <==



To date, the only way to argue {\em polynomial lower bounds} for dynamic algorithms is via {\em fine-grained complexity arguments}. These arguments rely on strong assumptions about {\em specific problems} such as the Strong Exponential Time Hypothesis (SETH) and the Online Matrix-Vector Multiplication Conjecture (OMv). While they have led to many exciting discoveries,  dynamic algorithms still miss out some benefits and lessons from the traditional ``coarse-grained'' approach that relates together classes of problems such as P and NP. In this paper we initiate the study of coarse-grained complexity theory for dynamic algorithms. Below are among questions that this theory can answer.

{\bf What if dynamic Orthogonal Vector (OV) is easy in the cell-probe model?} 
A research program for proving {\em polynomial unconditional lower bounds} for dynamic OV in the cell-probe model is motivated by the fact that many conditional lower bounds can be shown via reductions from the dynamic OV problem (e.g. [Abboud, V.-Williams, FOCS 2014]). 
Since the cell-probe model is more powerful than word RAM and has historically allowed smaller upper bounds (e.g. [Larsen, Williams, SODA 2017]), it might turn out that dynamic OV is easy in the cell-probe model, making this research direction infeasible. 
Our theory implies that if this is the case, there will be very interesting algorithmic consequences: If dynamic OV can be maintained in polylogarithmic worst-case update time in the cell-probe model, then so are several important dynamic problems such as $k$-edge connectivity,  $(1+\epsilon)$-approximate mincut, $(1+\epsilon)$-approximate matching, planar nearest neighbors, Chan's subset union and 3-vs-4 diameter. The same conclusion can be made when we replace dynamic OV by, e.g.,  subgraph connectivity, single source reachability, Chan's subset union, and 3-vs-4 diameter. 

{\bf Lower bounds for $k$-edge connectivity via dynamic OV?} The ubiquity of reductions from dynamic OV 

raises a question whether we can prove conditional lower bounds for, e.g., $k$-edge connectivity, approximate mincut, and approximate matching, via the same approach. Our theory provides a method to refute such possibility (the so-called {\em non-reducibility}). In particular, we show that there are no ``efficient'' reductions (in both cell-probe and word RAM models) from dynamic OV to $k$-edge connectivity under an assumption about the classes of dynamic algorithms whose analogue in the static setting is widely believed. 
We are not aware of any existing assumptions that can play the same role. (The NSETH of Carmosino et al. [ITCS 2016] is the closest one, but is not enough.)
To show similar results for other problems, one only need to develop efficient randomized {\em verification protocols} for such problems. 







\endinput




To date, the only way to argue polynomial lower bounds for dynamic algorithms is via {\em fine-grained complexity arguments}. These arguments rely on strong assumptions about {\em specific problems} such as the Strong Exponential Time Hypothesis (SETH) and the Online Matrix-Vector Multiplication Conjecture (OMv). While they have led to many exciting discoveries,  dynamic algorithms still miss out some benefits and lessons from the traditional ``coarse-grained'' approach that relates together classes of problems such as P and NP. In this paper we initiate the study of coarse-grained complexity theory for dynamic algorithms. Below are among questions that this theory can answer.

{\bf What if dynamic Orthogonal Vector (OV) is easy in the cell-probe model?} 
A research program for proving {\em polynomial unconditional lower bounds} for dynamic OV in the cell-probe model is motivated by the fact that many conditional lower bounds can be shown via reductions from the dynamic OV problem (e.g. [Abboud, V.-Williams, FOCS 2014]). 
Since the cell-probe model is more powerful than word RAM and has historically allowed smaller upper bounds (e.g. [Larsen, Williams, SODA 2017]), it might turn out that dynamic OV is easy in the cell-probe model, making this research direction infeasible. 
Our theory implies that if this is the case, there will be very interesting algorithmic consequences: If dynamic OV can be maintained in polylogarithmic worst-case update time in the cell-probe model, then so are several important dynamic problems such as $k$-edge connectivity,  $(1+\epsilon)$-approximate mincut, $(1+\epsilon)$-approximate matching, planar nearest neighbors, Chan's subset union and 3-vs-4 diameter. The same conclusion can be made when we replace dynamic OV by, e.g.,  subgraph connectivity, single source reachability, Chan's subset union, and 3-vs-4 diameter. 


{\bf Lower bounds for $k$-edge connectivity via dynamic OV?} The usefulness of reductions from dynamic OV in proving conditional lower bounds raises a question whether we can prove conditional lower bounds for, e.g., $k$-edge connectivity, approximate mincut, and approximate matching, via the same approach. Our theory provides a method to refute such possibility (the so-called {\em non-reducibility}). In particular, we show that there are no ``efficient'' reductions from dynamic OV to $k$-edge connectivity under an assumption about the classes of dynamic algorithms (namely, $\dPH \not\subseteq \dMA \cap \dcoMA$ which is widely believed for the static analogue). 
We are not aware of any existing assumptions that can play the same role. (The NSETH of Carmosino et al. [ITCS 2016] is the closest one, but is not enough.)
To show similar results for other problems, one only need to develop efficient randomized {\em verification protocols} for such problems. 





\endinput

=========================================
========================================




To date, the only way to rule out efficient {\em dynamic algorithms} (typically with polylogarithmic update time) is via {\em fine-grained complexity arguments}. These arguments rely on strong assumptions about {\em specific problems} such as the Strong Exponential Time Hypothesis (SETH) and the Online Matrix-Vector Multiplication Conjecture (OMv). While they have led to many exciting discoveries,  dynamic algorithms still miss out some benefits and lessons from the traditional ``coarse-grained'' approach that relates together classes of problems such as P and NP. For example, while refuting a coarse-grained assumption often means an exciting collapse of some complexity classes (e.g. P=NP), refuting SETH, OMv, or other assumptions has no known direct consequence to dynamic algorithms. Moreover, these conjectures often say nothing about the cell-probe model, the only model known to give unconditional lower bounds. 


In this paper, we show that some coarse-grained results can be obtained for dynamic algorithms in both word RAM and cell-probe models.  To start with, we define complexity classes $\dP$ and $\dNP$ for dynamic problems and show in both models that

\begin{quote}
	{\em if $\dP\neq \dNP$, then there is no ``efficient'' algorithms for many dynamic problems such as Subgraph connectivity, Single source reachability, Chan's subset union, and 3-vs-4 Diameter; otherwise, there are efficient algorithms for decision versions of many dynamic problems such as $k$-edge Connectivity, $(1+\epsilon)$-approximate Matching, Planar nearest neighbors, Chan's subset union and 3-vs-4 Diameter.}
\end{quote}

Here, ``efficient'' algorithms and the class $\dP$ are for deterministic algorithms with polylogarithmic worst-case update time in the standard cell-probe model. For word RAM, we have to relax the notion of efficient algorithms to allow quasi-polynomial preprocessing time and space. 


This result is obtained by defining the class $\dNP$ and polynomial hierarchy $\dPH$ with our notion of ``nondeterminism with rewards''. (This is, for example, different from the nondeterminism discussed by Husfeldt and Rauhe \cite{HusfeldtR03} and their follow-ups \cite{PatrascuD06,PatrascuThesis,Yin10,LarsenNonDeterministic,WangY14}.) This allows us to prove that (i) certain problems are $\dNP$-complete and  $\dNP$-hard, and (ii)  if $\dP=\dNP$ then $\dP=\dPH$, and thus many dynamic problems in $\dPH$ would admit efficient dynamic algorithms. Like in the static setting, the discussions can be extended to compare other complexity classes. One consequence is the following {\em non-reducibility} result.

\begin{quote}
	{\em if $\dPH \not\subseteq \dMA \cap \dcoMA$ (widely believed for the static analogue), then the $k$-edge connectivity problem is not $\dNP$-hard.}
\end{quote}

Consequently, there is no ``efficient'' (even randomized) reduction from the dynamic OV problem to $k$-edge connectivity. This rules out a common way to prove lower bounds based on SETH for $k$-edge connectivity. This opens a new direction to show non-reducibility for dynamic problems.  We are not aware of any existing conjectures that can play the same role. (The NSETH of Carmosino et al. [ITCS'16] is the closest one, but is not enough.)



\endinput




To date, the only way to rule out efficient {\em dynamic algorithms} (typically with polylogarithmic update time) is via {\em fine-grained complexity arguments}. These arguments rely on strong assumptions about {\em specific problems} such as the Strong Exponential Time Hypothesis (SETH) and the Online Matrix-Vector Multiplication Conjecture (OMv). While they have led to many exciting discoveries,  dynamic algorithms still miss out some benefits and lessons from the traditional ``coarse-grained'' approach that relates together classes of problems such as P and NP. 
For example, while refuting a coarse-grained assumption often means an exciting collapse of some complexity classes (e.g. P=NP),
refuting SETH, OMv, or other assumptions has no known direct consequence to dynamic algorithms.
Moreover, these conjectures often say nothing about the cell-probe model, the only model known to give unconditional lower bounds. 









In this paper, we show that some coarse-grained results can be obtained for dynamic algorithms in both word RAM and cell-probe models.  To start with, we define complexity classes $\dP$ and $\dNP$ for dynamic problems and show in both models that
\begin{quote}
	{\em if $\dP\neq \dNP$, then there is no ``efficient'' algorithms for many dynamic problems such as Subgraph connectivity, Single source reachability, Chan's subset union, and 3-vs-4 Diameter;
		otherwise, there are efficient algorithms for decision versions of many dynamic problems such as $k$-edge Connectivity, $(1+\epsilon)$-approximate Matching, Planar nearest neighbors, Chan's subset union and 3-vs-4 Diameter.}
\end{quote}
Here, ``efficient'' algorithms and the class $\dP$ are for deterministic algorithms with polylogarithmic worst-case update time in the standard cell-probe model. For word RAM, we have to relax the notion of efficient algorithms to allow quasi-polynomial preprocessing time and space. 

This result is obtained by defining the class $\dNP$ and polynomial hierarchy $\dPH$ with our notion of ``nondeterminism with rewards''. (This is, for example, different from the nondeterminism discussed by Husfeldt and Rauhe \cite{HusfeldtR03} and their follow-ups \cite{PatrascuD06,PatrascuThesis,Yin10,LarsenNonDeterministic,WangY14}.) This allows us to prove that (i) certain problems are $\dNP$-complete and  $\dNP$-hard,
and (ii)  if $\dP=\dNP$ then $\dP=\dPH$, and thus many dynamic problems in $\dPH$ would admit efficient dynamic algorithms. 
Like in the static setting, the discussions can be extended to compare other complexity classes, such as analogues of coNP, BPP, MA, and coMA. For example, we show that
\begin{quote}
	{\em if $\dPH \not\subseteq \dMA \cap \dcoMA$ (widely believed for the static analogue), then the $k$-edge connectivity problem is not $\dNP$-hard.}
\end{quote}
Consequently, there is no ``efficient'' (even randomized) reduction from the dynamic OV problem to $k$-edge connectivity (constructing such reduction is a common way to prove lower bounds based on SETH). This opens a new direction to show {\em non-reducibility} for dynamic problems.  We are not aware of any existing conjectures that can play the same role.
(The NSETH of Carmosino et al. [ITCS'16] is the closest one, but is not enough.)















\endinput





{\em Dynamic problems} concern whether one can quickly maintain some properties of an input data undergoing some {\em updates}. So far the only way to rule out efficient dynamic algorithms (typically with polylogarithmic update time) is via {\em fine-grained complexity arguments}, relying on strong assumptions about specific problems such as the Strong Exponential Time Hypothesis (SETH) and the Online Matrix-Vector Multiplication Conjecture (OMv). While this method has led to many exciting discoveries,  dynamic algorithms still miss out some benefits and lessons from the traditional ``coarse-grained'' approach that relates together classes of problems such as P and NP. For example, while refuting a coarse-grained conjecture (e.g. the $P\neq NP$ conjecture) often implies a collapse of problem classes and leads to exciting consequences (e.g. $P=NP$), there is no direct consequence to dynamic algorithms if SETH, OMv, or any other assumptions were refuted.
Moreover, these conjectures often say nothing about the cell-probe model, the only model known to give unconditional lower bounds. 







In this paper, we show that some coarse-grained results can be obtained for dynamic algorithms in both word RAM and cell-probe models when the notion of ``nondeterminism'' is carefully defined.  To start with, we define complexity classes $\dP$ and $\dNP$ and show in both models that
\begin{quote}
{\em if $\dP\neq \dNP$, then there is no ``efficient'' algorithms for many dynamic problems such as Subgraph connectivity, Single source reachability, Chan's subset union, and 3-vs-4 Diameter;
otherwise, there are efficient algorithms for decision versions of many dynamic problems such as $k$-edge Connectivity, $(1+\epsilon)$-approximate Matching, Planar nearest neighbors, Chan's subset union and 3-vs-4 Diameter.}
\end{quote}
Here, ``efficient'' algorithms and the class $\dP$ are for deterministic algorithms with polylogarithmic worst-case update time in the standard cell-probe model. For word RAM, we have to relax the notion of efficient algorithms to allow quasi-polynomial preprocessing time and space. 

This result is obtained by defining the class $\dNP$ and polynomial hierarchy $\dPH$ with our notion of ``nondeterminism with rewards''. (This is, for example, different from the nondeterminism discussed by Husfeldt and Rauhe \cite{HusfeldtR03} and their follow-ups \cite{PatrascuD06,PatrascuThesis,Yin10,LarsenNonDeterministic,WangY14}.) This allows us to prove that (i) certain problems are $\dNP$-complete and  $\dNP$-hard in the sense that if $\dP\neq \dNP$, then these problems do not admit efficient dynamic algorithms, and (ii)  if $\dP=\dNP$ then $\dP=\dPH$, and thus many dynamic problems in $\dPH$ would admit efficient dynamic algorithms. 
Like in the static setting, the discussions can be extended to compare other complexity classes, such as analogues of coNP, BPP, MA, and coMA. For example, we can show that in both word RAM and cell-probe models,
\begin{quote}
	{\em if $\dPH \not\subseteq \dMA \cap \dcoMA$ (which is believed for the static analogues), then $k$-edge connectivity is not $\dNP$-hard.}
\end{quote}
Consequently, there is no ``efficient'' (possibly randomized) reduction from the dynamic OV problem to $k$-edge connectivity, which is a typical way to prove lower bounds based on SETH. This opens a new direction as we are not aware of any existing conjectures that can rule out reductions in this manner.
(The NSETH of Carmosino et al. [ITCS'16] is the closest one, but is not enough at the current stage.)















\endinput


{\em Dynamic problems} concern whether one can quickly maintain some properties of an input data undergoing some {\em updates}. So far the only way to rule out efficient algorithms (typically with polylogarithmic update time) is via {\em fine-grained complexity arguments}, relying on strong assumptions such as the Strong Exponential Time Hypothesis (SETH) and the Online Matrix-Vector Multiplication Conjecture (OMv). While this method has led to many exciting discoveries,  dynamic algorithms still miss out some benefits from the traditional ``coarse-grained'' approach that relates together complexity classes such as P and NP. For example, unlike the static setting where proving and disproving P=NP will both lead to exciting consequences, there is no direct consequence to dynamic algorithms if SETH, OMv, or any other assumptions were refuted. 

In this paper, we show that some coarse-grained results can be obtained for dynamic algorithms in both word RAM and cell-probe models when the notion of ``efficient'' algorithms is slightly relaxed and ``nondeterminism'' is carefully defined.  To start with, we define complexity classes $\dP$ and $\dNP$ as analogues of P and NP for dynamic problems and show that 
\begin{enumerate}
	\item if $\dP\neq \dNP$, then there is no ``efficient'' algorithms for many dynamic problems such as Subgraph connectivity, Single source reachability, Chan's subset union, and 3-vs-4 Diameter;
	\item otherwise, there are  ``efficient'' algorithms for decision versions of many dynamic problems such as $k$-edge Connectivity, $(1+\epsilon)$-approximate Matching, Planar nearest neighbors, Chan's subset union and 3-vs-4 Diameter. 
\end{enumerate}
where ``efficient'' algorithms and the class $\dP$ are for deterministic algorithms with polylogarithmic worst-case update time and quasi-polynomial preprocessing time in the word RAM model or quasi-polynomial space in the cell-probe model. The quasi-polynomial complexity of algorithms in the second case is the cost we have to bear to discuss dynamic problems in the coarse-grained way; nevertheless, such algorithms should be intriguing already.\footnote{In particular, the second situation (when $\dP= \dNP$) will be more preferable if algorithms use polynomial preprocessing time in the word RAM model or polynomial space in the cell-probe model; nevertheless, we believe that algorithms with quasi-polynomial complexity would already be surprising.} 

This result is obtained by defining the class $\dNP$ and polynomial hierarchy $\dPH$ with our notion of ``nondeterminism with rewards''. (This is, for example, different from the nondeterminism discussed by Husfeldt and Rauhe \cite{HusfeldtR03} and their follow-ups \cite{PatrascuD06,PatrascuThesis,Yin10,LarsenNonDeterministic,WangY14}.) This allows us to prove that (i) certain problems are $\dNP$-complete and  $\dNP$-hard in the sense that if $\dP\neq \dNP$, then these problems do not admit efficient dynamic algorithms, and (ii)  if $\dP=\dNP$ then $\dP=\dPH$, and thus many dynamic problems in $\dPH$ would admit efficient dynamic algorithms. The discussions can be extended to other complexity classes, such as analogues of coNP, BPP, MA, coMA, and classes for promised problems.  


\endinput



{\em Dynamic problems} concern whether one can quickly maintain some properties of an input data undergoing some {\em updates}. So far the only way to rule out efficient algorithms (typically with polylogarithmic update time) is via {\em fine-grained complexity arguments}, relying on strong assumptions such as the Strong Exponential Time Hypothesis (SETH) and the Online Matrix-Vector Multiplication Conjecture (OMv). While this method has led to many exciting discoveries,  dynamic algorithms still miss out some benefits from the traditional ``coarse-grained'' approach that relates together complexity classes such as P and NP. For example, unlike the static setting where proving and disproving P=NP will both lead to exciting consequences, there is no direct consequence to dynamic algorithms if SETH, OMv, or any other assumptions were refuted. 

In this paper, we show that some coarse-grained results can be obtained for dynamic algorithms in both word RAM and cell-probe models when the notion of ``efficient'' algorithms is slightly relaxed and ``nondeterminism'' is carefully defined.  To start with, we define complexity classes $\dP$ and $\dNP$ as analogues of P and NP for dynamic problems and show that 
\begin{enumerate}
	\item if $\dP\neq \dNP$, then there is no ``efficient'' algorithms for many dynamic problems such as Subgraph connectivity, Single source reachability, Chan's subset union, and 3-vs-4 Diameter;
	\item otherwise, there are  ``efficient'' algorithms for decision versions of many dynamic problems such as $k$-edge Connectivity, $(1+\epsilon)$-approximate Matching, Planar nearest neighbors, Chan's subset union and 3-vs-4 Diameter. 
\end{enumerate}
where ``efficient'' algorithms and the class $\dP$ are for deterministic algorithms with polylogarithmic worst-case update time and quasi-polynomial preprocessing time in the word RAM model or quasi-polynomial space in the cell-probe model. The quasi-polynomial complexity of algorithms in the second case is the cost we have to bear to discuss dynamic problems in the coarse-grained way; nevertheless, such algorithms should be intriguing already.\footnote{In particular, the second situation (when $\dP= \dNP$) will be more preferable if algorithms use polynomial preprocessing time in the word RAM model or polynomial space in the cell-probe model; nevertheless, we believe that algorithms with quasi-polynomial complexity would already be surprising.} 

This result is obtained by defining the class $\dNP$ and polynomial hierarchy $\dPH$ with our notion of ``nondeterminism with rewards''. (This is, for example, different from the nondeterminism discussed by Husfeldt and Rauhe \cite{HusfeldtR03} and their follow-ups \cite{PatrascuD06,PatrascuThesis,Yin10,LarsenNonDeterministic,WangY14}.)
This allows us to prove that (i) certain problems are $\dNP$-complete and  $\dNP$-hard in the sense that if $\dP\neq \dNP$, then these problems do not admit efficient dynamic algorithms, and (ii)  if $\dP=\dNP$ then $\dP=\dPH$, and thus many dynamic problems in $\dPH$ would admit efficient dynamic algorithms.
The discussions can be extended to other complexity classes, such as analogues of coNP, BPP, MA, coMA, and classes for promised problems.  

\endinput




{\em Dynamic problems} concern whether one can quickly maintain some properties of an input data undergoing some {\em updates}. So far the only way to rule out efficient algorithms (typically with polylogarithmic update time) is via {\em fine-grained complexity arguments}, relying on strong assumptions such as the Strong Exponential Time Hypothesis (SETH) and the Online Matrix-Vector Multiplication Conjecture (OMv). While this method has led to many exciting discoveries,  dynamic algorithms still miss out some benefits from the traditional ``coarse-grained'' approach that relates together complexity classes such as P and NP. For example, unlike the static setting where proving and disproving P=NP will both lead to exciting consequences, there is no direct consequence to dynamic algorithms if SETH, OMv, or any other assumptions were refuted. 

In this paper, we show that some coarse-grained results can be obtained for dynamic algorithms in both word RAM and cell-probe models when the notion of ``efficient'' algorithms is slightly relaxed and ``nondeterminism'' is carefully defined. 
To start with, we define complexity classes $\dP$ and $\dNP$ as analogues of P and NP for dynamic problems and show that 
\begin{enumerate}
	\item if $\dP\neq \dNP$, then there is no ``efficient'' algorithms for many dynamic problems such as Subgraph connectivity, Single source reachability, Chan's subset union, and 3-vs-4 Diameter;
	\item otherwise, there are  ``efficient'' algorithms for decision versions of many dynamic problems such as $k$-edge Connectivity, $(1+\epsilon)$-approximate Matching, Planar nearest neighbors, Chan's subset union and 3-vs-4 Diameter. 
\end{enumerate}
where ``efficient'' algorithms and the class $\dP$ are for deterministic algorithms with polylogarithmic worst-case update time and quasi-polynomial preprocessing time in the word RAM model or quasi-polynomial space in the cell-probe model. The quasi-polynomial complexity of algorithms in the second case is the cost we have to bear to discuss dynamic problems in the coarse-grained way; nevertheless, such algorithms should be intriguing already.\footnote{In particular, the second situation (when $\dP= \dNP$) will be more preferable if algorithms use polynomial preprocessing time in the word RAM model or polynomial space in the cell-probe model; nevertheless, we believe that algorithms with quasi-polynomial complexity would already be surprising, and some of these results would in fact contradict SETH.} 

This result is obtained by defining the class $\dNP$ and {\em polynomial hierarchy} $\dPH$ with a notion of nondeterminism (it, for example, differs from the nondeterminism discussed by Husfeldt and Rauhe \cite{HusfeldtR03} and their follow-ups \cite{PatrascuD06,PatrascuThesis,Yin10,LarsenNonDeterministic,WangY14}).
This allows us to prove that (i) certain problems are $\dNP$-complete and  $\dNP$-hard in the sense that if $\dP\neq \dNP$, then these problems do not admit efficient dynamic algorithms, and (ii)  if $\dP=\dNP$ then $\dP=\dPH$, and thus many dynamic problems in $\dPH$ would admit efficient dynamic algorithms.
The discussions can be extended to other complexity classes, such as analogues of coNP, BPP, MA, coMA, and classes for promised problems.  



\endinput







{\em Dynamic problems} concern whether one can quickly maintain some properties of an input data undergoing some {\em updates}. So far the only way to rule out efficient algorithms (typically with polylogarithmic update time) is via {\em fine-grained complexity arguments}, relying on strong assumptions such as the Strong Exponential Time Hypothesis (SETH) and the Online Matrix-Vector Multiplication Conjecture (OMv). While this method has led to many exciting discoveries, 
dynamic algorithms still miss out some benefits provided by the traditional ``coarse-grained'' approach that relates together complexity classes such as P and NP. 
For example, unlike the static setting where proving and disproving P=NP will both lead to exciting consequences, there is no direct consequence to dynamic algorithms if SETH, OMv, or any other assumptions were refuted. 



In this paper, we show that some coarse-grained results can be obtained for dynamic algorithms when the notion of ``efficient'' algorithms is slightly relaxed and the notion of ``nondeterminism'' is slightly restricted. 
To start with, we define complexity classes $\dP$ and $\dNP$ as analogues of P and NP for dynamic problems and show that 
\begin{enumerate}
	\item if $\dP\neq \dNP$, then there is no ``efficient'' algorithms for many dynamic problems such as Subgraph connectivity, Single source reachability, Chan's subset union, and 3-vs-4 Diameter; 
	\item otherwise, there are  ``efficient'' algorithms for decision versions of many dynamic problems such as $k$-edge Connectivity, $(1+\epsilon)$-approximate Matching, Planar nearest neighbors, Chan's subset union and 3-vs-4 Diameter, 
\end{enumerate}
where ``efficient'' refer to deterministic algorithms with polylogarithmic worst-case update time and quasi-polynomial preprocessing time in the RAM model or quasi-polynomial space in the cell-probe model. The latter quasi-polynomial complexity is the cost we currently have to pay to 
obtain results like in static coarse-grained complexity.\footnote{In particular, the second situation (when $\dP= \dNP$) will be nicer if algorithms use polynomial preprocessing time or space; nevertheless, we believe that such algorithm will already be surprising.} 

This result is obtained by defining the class $\dNP$ and {\em polynomial hierarchy} $\dPH$ with a careful notion of nondeterminism; for example, in the cell-probe model it can be viewed as a restricted version of nondeterminism discussed by Husfeldt and Rauhe \cite{HusfeldtR03} and the follow-ups \cite{patrascu2006logarithmic,patrascu2004lower,Yin10,LarsenNonDeterministic,WangY14}.
This allows us to (i) identify $\dNP$-complete and -hard problems in the sense that if $\dP\neq \dNP$, then these problems do not admit efficient dynamic algorithms, and (ii)  just like in the static setting, if $\dP=\dNP$ then $\dP=\dPH$, and thus many dynamic problems in $\dPH$ will admit efficient dynamic algorithms. 
We can extend the discussions to other complexity classes, such as the analogues of coNP and BPP. 


\endinput








{\em Dynamic problems} concern whether one can quickly maintain some properties of an input data undergoing some {\em updates}. So far the only way to rule out efficient algorithms (typically with polylogarithmic update time) is via {\em fine-grained complexity arguments}, relying on strong assumptions such as the Strong Exponential Time Hypothesis (SETH) and the Online Matrix-Vector Multiplication Conjecture (OMv). While this method has led to many exciting discoveries, 
dynamic algorithms still miss out some benefits provided by the traditional ``coarse-grained'' approach that relates together complexity classes such as P and NP. 
For example, unlike the static setting where proving and disproving P=NP will both lead to exciting consequences, there is no direct consequence to dynamic algorithms if SETH, OMv, or any other assumptions were refuted. 

In this paper, we show that many coarse-grained arguments for static algorithms can be extended to discuss dynamic algorithms under some relaxations, i.e. either algorithms in the RAM model with quasi-polynomial preprocessing time or those in the cell-probe model with quasi-polynomial space. To start with, in one of our main results we define complexity classes $\dP$ and $\dNP$ as analogues of P and NP for dynamic problems and show that 
\begin{enumerate}
	\item if $\dP\neq \dNP$, then there is no worst-case polylogarithmic-update-time algorithm for many dynamic problems such as ..., even with quasi-polynomial preprocessing time;
	\item otherwise, many dynamic problems such as ... admit worst-case polylogarithmic-update-time algorithms with quasi-polynomial preprocessing time.
\end{enumerate}
The above result also holds in the cell-probe model with the term ``quasi-polynomial preprocessing time'' replaced by ``quasi-polynomial space''. 



The drawback ...
Should talk about drawback? Will talk about techniques...

** Two tricks: Pay preprocessing + protocol as optimization problem. 


\endinput






{\em Dynamic problems} concern whether one can quickly maintain some properties of an input data undergoing some {\em updates}. 
So far the only way to argue against efficient algorithms (typically with polylogarithmic update time) is via {\em fine-grained complexity arguments}, relying on strong assumptions such as the Strong Exponential Time Hypothesis (SETH) and the Online Matrix-Vector Multiplication Conjecture (OMv).
While this method has led to many exciting discoveries, it does not provide all benefits provided by the traditional ``coarse-grained'' approach, which tries to relate together complexity classes such as P and NP. For example, there is no direct consequence to dynamic algorithms if SETH, OMv, or any other assumptions are false; this is unlike the static setting where the traditional complexity theory shows that proving and disproving P=NP will both lead to exciting consequences. 





In this paper, we explore a traditional approach in the static setting centering around the notions of nondeterminism and completeness. We define complexity classes $\dP$ and $\dNP$ as analogues of P and NP for dynamic problems and show that 



\begin{enumerate}
	\item if $\dP\neq \dNP$, then there is no worst-case polylogarithmic-update-time algorithm for many dynamic problems such as ..., even with quasi-polynomial preprocessing time;
	\item otherwise, there will  
\end{enumerate}


 in the bit-probe model (where the time denotes the number of memory accesses).\footnote{Since we do not focus on the precise time, it does not make much difference whether one consider bit-probe or cell-probe models (where each cell is typically of size $O(\log n)$); in particular  $\dP$ and $\dNP$ remain the same. Note that we only consider the worst-case update time in this paper, and not the amortized one.}  









{\em Dynamic problems} concern whether one can quickly maintain some properties of an input data undergoing some {\em updates}. So far, popular ways to argue about their difficulties have been to either (i) prove information-theoretic lower bounds in the cell- or bit-probe models or (ii) prove conditional lower bounds based on various assumptions. In this paper, we explore a traditional approach in the static setting centering around the notions of nondeterminism and completeness. 
We establish an analogue of NP-completeness for dynamic problems in the bit- or cell-probe models, and use it to explain the hardness of various dynamic problems.




In more details, consider {\em polynomial-time} dynamic algorithms as those that can handle each update in time polynomial {\em in the update size}. %
This captures the sought-for update time for many dynamic problems, such as the polylogarithmic update time for graphs undergoing edge updates.  
With this notion, one can define $\dP$ and $\dNP$ as analogues of P and NP for dynamic problems in the bit-probe model (where the time denotes the number of memory accesses).\footnote{Since we do not focus on the precise time, it does not make much difference whether one consider bit-probe or cell-probe models (where each cell is typically of size $O(\log n)$); in particular  $\dP$ and $\dNP$ remain the same. Note that we only consider the worst-case update time in this paper, and not the amortized one.}  
The complexity class at the center of our study is called $\drankNP$, which is an analogue of NP in the bit-probe model with some mild restrictions. It is a huge class that includes a number of natural and hard dynamic problems, such as connectivity, approximate matching, planar nearest neighbor, and triangle detection. 

Our main result is that a problem called {\em dynamic narrow DNF evaluation} is $\drankNP$-complete in the sense that it is in $\drankNP$ and if it is in $\dP$, 
then so are all problems in $\drankNP$. Since it turns out that dynamic DNF evaluation is equivalent to a dynamic version of the Orthogonal Vector problem, it follows that many natural dynamic graph problems such as approximate diameter, subgraph connectivity, maximum flow, and in fact all problems proven to be SETH-hard by Abboud and V.-Williams [FOCS 2014], are $\drankNP$-hard. In other words, unless $\dP=\drankNP$, these problems do not admit polynomial-time dynamic algorithms in the bit-probe model (thus in the RAM model as well). 
In the RAM model, the same can be proven for algorithms with large enough preprocessing time and space, and additionally lower bounds for dynamic DNF evaluation can be proven from SETH and the OMv conjecture.





\endinput







{\em Dynamic problems} concern whether one can quickly maintain some properties of an input data undergoing some {\em updates}. So far, popular ways to argue about their difficulties have been to either (i) prove information-theoretic lower bounds in the cell- or bit-probe models or (ii) prove conditional lower bounds based on various assumptions. In this paper, we explore a traditional approach in the static setting centering around the notions of nondeterminism and completeness. 
We show that it is possible to prove and get new insights from an analogue of NP-completeness, when considered in the dynamic cell- or bit-probe models.






In more details, consider {\em polynomial-time} dynamic algorithms as those that can handle each update in time polynomial {\em in the update size}. This generalizes the notion of polynomial time for static problems and captures the sought-for update time for many dynamic problems, such as the polylogarithmic update time for graphs undergoing edge updates.  
With this notion, one can define $\dPprb$, $\dNPprb$ and $\dcoNPprb$ as analogues of P, NP and coNP for dynamic problems in the bit-probe model (where the time denotes the number of memory accesses).\footnote{Since we do not focus on the precise time, it does not make much difference whether one consider bit-probe or cell-probe models (where each cell is typically of size $O(\log n)$). Note that we only consider the worst-case update time in this paper, and not the amortized one.}  
The complexity class at the center of our study is called $\drankNPprb$, which is an analogue of NP in the bit-probe model with some mild restrictions. It is a huge class that includes a number of natural and hard dynamic problems, such as connectivity, approximate matching, and logarithmic-size clique detection under edge deletions. 

Our main result is that a problem called {\em dynamic DNF evaluation} is $\drankNPprb$-complete in the sense that it is in $\drankNPprb$ and if it is in $\dPprb$, 
then so are all problems in $\drankNPprb$. Since it turns out that dynamic DNF evaluation is equivalent to a dynamic version of the Orthogonal Vector problem, it follows that many natural dynamic graph problems such as approximate diameter, subgraph connectivity, maximum flow, and in fact most problems proven to be SETH-hard by Abboud and V.-Williams [FOCS 2014], are $\drankNPprb$-hard. In other words, unless $\dPprb=\drankNPprb$, these problems do not admit polynomial-time dynamic algorithms in the bit-probe model (thus in the RAM model as well). 
In the RAM model, the same can be proven for algorithms with large enough preprocessing time. 




\endinput

\medskip

{\em Dynamic problems} concern whether one can quickly maintain some properties of an input data undergoing some {\em updates}. So far, popular ways to argue about their difficulties has been to either (i) prove information-theoretic lower bounds in the cell- or bit-probe models or (ii) prove conditional lower bounds based on various assumptions. In this paper, we explore a traditional approach from the static setting, where we define analogues of complexity classes such as P, NP, and coNP, and prove completeness for these classes. We show that this can be done and can give new insights to the difficulties of dynamic problems, when done in the cell- or bit-probe models. 


In more details, consider a natural notion of {\em polynomial-time dynamic algorithms}, referring to algorithms that take time polynomial in the {\em update size} to handle each update. 
This generalizes the notion of polynomial time for static problems and captures the sought-for update time for many dynamic problems, such as the polylogarithmic update time for graphs undergoing edge updates.  
With this notion, one can define analogues of P, NP, coNP, etc., and a natural question arise: {\em can one identify and make use of NP-complete problems as in the static setting?}


In this paper, we show that this is possible if we focus on the number of probes rather than the actual time complexity, and by considering a fairly big complexity class lying between the dynamic analogues of P and NP, called $\drankNP$. In particular, we show that a problem of maintaining whether a DNF formula is true under the change of variables' values 




\footnote{Since we do not focus on the precise time, it does not make much difference whether one consider bit-probe or cell-probe models (where each cell is typically of size $O(\log n)$). Note that the definition of $\dP$ only consider the worst-case update time, and not the amortized one.}  






\endinput








we define complexity classes such as $\dP$, $\dNP$ and $\dcoNP$ for dynamic problems, where the time efficiency is measured on the {\em bit-probe} model and against the {\em update size} instead of the input size
They are meant to be natural counterparts of complexity classes P, NP, and coNP for static problems; for example, for the case of dynamic graph problems with edge updates, $\dP$ include problems at admit algorithms with polylogarithmic update time -- the sought-for bound for most dynamic graph problems -- and $\dNP$ include problems that are not yet known to have such time, such as 






\endinput



In particular, we define complexity classes such as $\dP$, $\dNP$ and $\dcoNP$ for dynamic problems, where the time efficiency is measured on the {\em bit-probe} model and against the {\em update size} instead of the input size\footnote{Since we do not focus on the precise time, one can equivalently define the class on the cell-probe model where each cell is of size $O(\log n)$. Note that the definition of $\dP$ only consider the worst-case update time, and not the amortized one.}. 
They are meant to be natural counterparts of complexity classes P, NP, and coNP for static problems; for example, for the case of dynamic graph problems with edge updates, $\dP$ include problems at admit algorithms with polylogarithmic update time -- the sought-for bound for most dynamic graph problems -- and $\dNP$ include problems that are not yet known to have such time, such as 








In particular, we define the complexity class $\dP$ as the class of dynamic problems such that we can handle each update in time {\em polynomial in the update size}, where the time measures the number of probes in the bit-probe model.\footnote{Since we do not focus on the precise time, one can equivalently define the class on the cell-probe model where each cell is of size $O(\log n)$. Note that the definition of $\dP$ only consider the worst-case update time, and not the amortized one.} 
This class is meant to be an analogue of the class P from the static setting, and for many problems falling into this class means admitting efficient algorithms that have been long sought for; for example, if a dynamic graph problem under edge updates is in $\dP$, then it admits a deterministic algorithm with polylogarithmic worst-case update time in the probe model.  



 $\dNP$, $\dcoNP$ for dynamic problems. They are meant to be natural counterparts of complexity classes for static problems, such as  P, NP, and coNP, with the main difference being the efficiency defined on the update size, not the input size, and the complexity measured in the {\em bit-probe} model. We then define a subclass 



 The {\em complexity theoretic} approach, which has been successful in classifying {\em static problems} based on their inherent difficulties and relating those classes together, has not seen much success in understanding dynamic problems. 



\endinput


{\em Dynamic problems} concern whether one can quickly maintain some properties of an input data undergoing some {\em updates}. So far, popular ways to argue about their difficulties has been to either (i) prove (rather small) information-theoretic lower bounds in the cell-probe model or (ii) prove conditional lower bounds based on various assumptions. The {\em complexity theoretic} approach, which has been successful in classifying {\em static problems} based on their inherent difficulties and relating those classes together, has not seen much success in understanding dynamic problems. 



In this paper, we show that this approach, when studied in the {\em bit-probe model}, can give new insights to the difficulties of dynamic problems; for example, we show that many natural dynamic graph problems such as approximate diameter, subgraph connectivity, maximum flow, and in fact most SETH-hard problems, are {\em hard} for a big class of problems called $\drankNP$, in the sense that if any of them can be maintained with polylogarithmic update time in the bit-probe model, then so do all other problems in $\drankNP$. 


More precisely, we define complexity classes such as $\dP$, $\dNP$, $\dcoNP$ for dynamic problems. They are meant to be natural counterparts of complexity classes for static problems, such as  P, NP, and coNP, with the main difference being the efficiency defined on the update size, not the input size, and the complexity measured in the {\em bit-probe} model. We then define a subclass 











\endinput


In particular, we define complexity classes such as $\dP$, $\dNP$, $\dcoNP$ for dynamic problems. They are meant to be natural counterparts of complexity classes for static problems, such as  P, NP, and coNP, with the main difference being the efficiency defined on the update size, not the input size, and the complexity measured in the {\em bit-probe} model. For example, all dynamic graph problems with worst-case polylogarithmic update time are in $\dP$. 





; for example, we can show that natural graph problems such as reachability is hard . In particular, we define  





Whether one can quickly maintain some properties of an input data undergoing some {\em updates} is a major research question in computer science and in particular the area of {\em dynamic algorithms}. Popular ways to answer this question has been so far to prove either (i) information-theoretic lower bounds in the cell-probe model or (ii) conditional lower bounds based on popular conjectures.
The {\em complexity theoretic} approach, which has been successful in classifying {\em static problems} based on their inherent difficulty, and relating those classes to each other, has not seen much success in understanding dynamic problems. 


... is possible and could give new insights ...  




==> acknowledgment.tex <==
\section*{Acknowledgment}

This project has received funding from the European Research Council (ERC) under the European
Unions Horizon 2020 research and innovation programme under grant agreement No 715672. Danupon
Nanongkai and Thatchaphol Saranurak were also partially supported by the Swedish Research Council (Reg. No. 2015-04659).



==> contributions.tex <==
\section{Our Contributions in Details} 
\label{sec:intro:contribution}





We show that coarse-grained complexity results similar to the static setting can be obtained for dynamic problems in the bit-probe/cell-probe model of computation,\footnote{Throughout the paper, we use the cell-probe and bit-probe models interchangeably since the complexity in these models are the same up to polylogarithmic factors.}   provided the notion of ``nondeterminism'' is carefully defined.\footnote{We do not consider the Turing machine because it is not suitable for implementing dynamic algorithms (since we cannot access an arbitrary tape location in $O(1)$ time). There is no efficient algorithm even for a basic data structure like the binary search tree.}  Recall that the cell-probe model is similar to the word RAM model, but the time complexity is measured by the number of memory reads and writes (probes); other operations are free (see \Cref{sec:model:dynamic}). 
Like in the static setting, we only consider {\em decision} dynamic problems,\footnote{Our results extend naturally to {\em promised problems} which are useful when we discuss approximation algorithms. We do not discuss promised problems here to keep the discussions simple.} meaning that the output after each update is either ``yes'' or ``no''.\repOblivious\xspace





We start with our main results which can be obtained with 
appropriate definitions of complexity classes $\dP \subseteq \dNP \subseteq \dPH$ for dynamic problems:
These classes are described after \Cref{thm:intro:results_summary}.  For now they should be thought of as analogues of the classes P, NP and PH (polynomial hierarchy). 
\begin{theorem}($\dP$ vs. $\dNP$) \label{thm:intro:results_summary} Below, the phrase ``efficient algorithms'' refer to dynamic algorithms that are deterministic and require  polylogarithmic worst-case update time and  polynomial space to handle a polynomial number of updates in the bit-probe/cell-probe model: 
\begin{enumerate}[noitemsep]
	\item \label{item:NP-hard-problems} The dynamic orthogonal vector (OV) problem is ``$\dNP$-complete", and there are a number of dynamic problems that are ``$\dNP$-hard'' in the sense that if $\dP\neq \dNP$, then they admit {\em no} efficient algorithms.
	These problems include decision versions of Subgraph connectivity, ST-reachability, Chan's subset union,  and 3-vs-4 Diameter (see \Cref{table:BPP-NP,table:NP hard} for more).
	\item \label{item:PH-problems} If $\dP=\dNP$ then $\dP=\dPH$, meaning that all problems in $\dPH$ (which contains the class $\dNP$) admit efficient algorithms. These problems include decision versions of $k$-edge Connectivity, $(1+\epsilon)$-approximate Matching,\footnote{Technically speaking, $(1+\epsilon)$-approximate matching is a {\em promised} or {\em gap} problem in the sense that for some input instance all answers are correct. It is in $\dprmPH$ which is bigger than $\dPH$. We can make the same conclusion for promised problems: If $\dP=\dNP$, then all problems in $\dprmPH$ admit efficient algorithms.} $(1+\epsilon)$-approximate mincut, Planar nearest neighbors, Chan's subset union and 3-vs-4 Diameter (see \Cref{table:BPP-NP,table:PH} for more). 
	
\end{enumerate}
Thus, proving or disproving $\dP\neq \dNP$ will both lead to interesting consequences: If $\dP\neq \dNP$, then many dynamic problems do not admit efficient algorithms. Otherwise, if $\dP = \dNP$, then many problems  admit efficient algorithms which are not known or even believed to exist.
\end{theorem}

















As another showcase, our study implies a way to show {\em non-reducibility}, like below. 

\begin{theorem}\label{thm:intro:ruleout_reductions}
Assuming  $\dPH \not\subseteq \dMA \cap \dcoMA$, the $k$-edge connectivity problem cannot be $\dNP$-hard.  Consequently, there is no ``efficient reduction'' from the dynamic Orthogonal Vector (OV) problem to $k$-edge connectivity. 
\end{theorem}




From the discussion in \Cref{sec:intro}, recall that the $k$-edge connectivity problem is currently known to admit a polylogarithmic amortized update time algorithm for $k\leq 2$, and a $O(\sqrt{n}\polylog (n))$ update time algorithm for $k\in [3, O(\log n)].$

It is a very important open problem whether it admits polylogarithmic worst-case update time. \Cref{thm:intro:ruleout_reductions} rules out a way to prove lower bounds and suggest that an efficient algorithm might exist. 

A more important point beyond the $k$-edge connectivity problem is that one can prove a similar result for any dynamic problem $X$ by showing that  $X\in  \dMA \cap \dcoMA$ or, even better, $X\in  \dNP \cap \dcoNP$. (See \Cref{sec:open} for some candidates of $X$.)
This is easier than showing a dynamic algorithm for $X$ itself. Thus, this method is an example of the by-products of our study that we expect to be useful for developing algorithms and lower bounds for dynamic problems in  future. See \Cref{sec:contribution:other:results} and \Cref{part:connectivity} for more details. 
As noted in \Cref{sec:intro}, we are not aware of any  existing technique 
 
that is capable of deriving a non-reducibility result of this kind. 








The key challenge in deriving the above results is to come up with the right set of definitions for  various dynamic complexity classes. 
 We provide some of these definitions and discussions here, but defer more details to later in the paper.  


\subsection{Defining the Complexity Classes $\dP$ and $\dNP$}
\label{sec:contribution:classes}

\noindent {\bf Class $\dP$.}
We start with $\dP$, the class of dynamic problems that admit ``efficient'' algorithms in the cell-probe model.  

For any dynamic problem, define its {\em update size} to be the number of bits needed to describe each update.	Note that we have not yet defined what dynamic problems are formally. Such a definition is needed for a proper, rigorous  description of our complexity classes, and can be found later in the paper (see~\ref{sec:model} for more details). For an intuition, it suffices to keep in mind that most dynamic graph problems -- where each update is an edge deletion or insertion -- have logarithmic update size (since it takes $O(\log n)$ bits to specify an edge in an $n$-node graph).

\begin{defn}[$\dP$; brief]\label{def:intro:dP}
A dynamic problem with polylogarithmic update size is in $\dP$ if it admits a deterministic algorithm with polylogarithmic worst-case update time for handling a sequence of polynomially many updates.\repQuasi
\end{defn}

Examples of problems in $\dP$ include connectivity on plane graphs and predecessor; for more, see \Cref{table:P}. 
Note that one can define $\dP$ more generally to include problems with larger update sizes. Our complexity results hold even with this more general definition. However, since our results are most interesting for problems with polylogarithmic update size, we focus on this case in this paper to avoid cumbersome notations. 


\paragraph{Class $\dNP$ and nondeterminism with rewards.}
Next, we introduce our complexity class $\dNP$. Recall that in the static setting the class NP consists of the set of problems that admit efficiently verifiable proofs or, equivalently, that are solvable in polynomial time by a nondeterministic algorithm. 
Our notion of nondeterminism is captured by the proof-verification definition where, after receiving  a proof, the verifier does not only output YES/NO, but also a {\em reward}, which is supposed to be maximized  at every step. 


Before defining $\dNP$ more precisely, we remark that the notion of reward is a key for our $\dNP$-completeness proof. Having the constraint about rewards potentially makes $\dNP$ contains less problems.  Interestingly, all natural problems that we are aware of remains in $\dNP$ even with this constraint. This might not be a big surprise, when it is realized that in the static setting imposing a similar constraint about the reward does {\em not} make the class (static) NP smaller; see more discussions below.
We now define $\dNP$ more precisely.
\begin{defn}[$\dNP$; brief]\label{def:intro:dNP}
	A dynamic problem $\Pi$ with polylogarithmic update size is in $\dNP$ if there is a verifier\repQuasi{} that can do the following over a sequence of  polynomially many updates:
	(i) after every update, the verifier takes the update and a polylogarithmic-size {\em proof} as an input, and
	(ii) after each update, the verifier outputs in polylogarithmic time a pair $(x, y)$, where $x\in \{YES,NO\}$ and $y$ is an integer (representing a reward) with the following properties.\footnote{Later in the paper, we use $x=1$ and $x=0$ to represent $x=YES$ and $x=NO$, respectively.}
	\begin{enumerate}[noitemsep]
		\item If the current input instance is an YES-instance and the verifier has so far always received a proof that maximizes the reward at every step, then the verifier outputs $x=YES$.
		\item If the current input instance is a NO-instance, then the verifier outputs $x=NO$  regardless of the sequence of proofs it has received so far. \qedhere
	\end{enumerate}
\end{defn} 

To digest the above definition, first consider the {\em static}  setting. One can redefine the class NP for static problems in a similar fashion to \Cref{def:intro:dNP} by removing the preprocessing part and letting  the only update be the whole input. Let us refer to this new (static) complexity class as ``{\em reward-NP}''.
To show that a static problem is in reward-NP, a verifier has to output some reward in addition to the YES/NO answer. Since usually a proof received in the static setting is a solution itself, a natural choice for reward is the {\em cost} of the solution (i.e., the proof). For example, a ``proof'' in the maximum clique problem is a big enough clique, and in this case an intuitive reward would be the size of the clique given as a proof. Observe that this is sufficient to show that max clique is in reward-NP. In fact, it turns out that {\em in the static setting the complexity classes NP and reward-NP are equal}.\footnote{Let $\Pi$ be any problem in the original static NP and $V$ be a corresponding verifier. We extend $V$ to $V'$  which outputs $x=YES/NO$ as $V$ and outputs $y=1$ as a reward if $x=YES$ and $y=0$ otherwise. It is not hard to check that $V'$ satisfies conditions in \Cref{def:intro:dNP}.} To further clarify~\ref{def:intro:dNP},  we now consider examples of some well-known dynamic problems that happen to be in $\dNP$. 






\begin{example}[Subgraph Detection]\label{ex:subgraphDetect_inNP}
In the {\em dynamic subgraph detection} problem, an $n$-node and $k$-node graphs $G$ and $H$ are given at the preprocessing, for some $k=\polylog(n)$.  Each update is an edge insertion or deletion in $G$. We want an algorithm to output YES if and only if $G$  has $H$ as a subgraph. 

This problem is in $\dNP$ due to the following verifier: the verifier outputs $x=YES$ if and only if the proof (given after each update) is a mapping of the edges in $H$ to the edges in a subgraph of $G$ that is isomorphic to $H$. With output $x=YES$, the verifier gives  reward $y=1$. With output $x=NO$, the verifier gives reward $y=0$.  Observe that the proof  is of polylogarithmic size (since $k = \polylog (n))$, and the verifier can calculate its outputs $(x,y)$ in polylogarithmic time. Observe further that the properties stated in \Cref{def:intro:dNP} are satisfied: if the current input instance is a YES-instance, then the reward-maximizing proof is a mapping between $H$ and the subgraph of $G$ isomorphic to $H$, causing the verifier to output $x=YES$; otherwise, no proof will make the verifier output $x=YES$.  
\end{example}


The above example is in fact too simple to show the strength of our definition that allows $\dNP$ to include many natural problems (for one thing, $y$ is simply 0/1 depending on $x$). 
The next example demonstrates how the definition allows us to develop more sophisticated verifiers for other problems. 






\begin{example}[Connectivity]\label{ex:intro:connectivity in NP}
In the {\em dynamic connectivity} problem, an $n$-node graph $G$ is given at the preprocessing.  Each update is an edge insertion or deletion in $G$. We want an algorithm to output YES if and only if $G$ is connected. 

This problem is in $\dNP$ due to the following verifier. After every update, the verifier   maintains a forest $F$ of $G$. A proof (given after each update) is an edge insertion to $F$ or an $\bot$ symbol indicating that there is no update to $F$.  It handles each update as follows.

\begin{itemize}[noitemsep]
	\item After an edge $e$ is inserted into $G$, the verifier checks if $e$ can be inserted into $F$ without creating a cycle. This can be done in $O(\polylog(n))$ time using a link/cut tree data structure \cite{SleatorT81}. It outputs reward $y=0$. (No proof  is needed in this case.)
	\item After an edge $e$ is deleted from $G$,  the verifier checks if $F$ contains $e$. If not, it outputs  reward $y=0$ (no proof  is needed in this case). If $e$ is in $F$, the verifier reads the proof (given after $e$ is deleted). If the proof is $\bot$ it outputs reward $y=0$. Otherwise, let the proof be an edge $e'$. The verifier checks if $F'=F\setminus\{e\}\cup \{e'\}$ is a forest; this can be done in $O(\polylog(n))$ time using a link/cut tree data structure \cite{SleatorT81}. If $F'$ is a forest, the verifier sets $F\gets F'$ and outputs reward $y=1$; otherwise, it outputs reward $y=-1$.  
\end{itemize}
After each update, the verifier outputs $x=YES$ if and only if $F$ is a spanning tree of $G$.

Observe that if the verifier gets a proof that maximizes the reward after every update, the forest $F$ will always be a spanning forest (since inserting an edge $e'$ to $F$ has higher reward than giving $\bot$ as a proof). Thus, the verifier will always output $x=YES$ for YES-instances in this case. It is not hard to see that the verifier never outputs $x=YES$ for NO-instances, no matter what proof it receives. 
\end{example}





In short, a proof for the connectivity problem is the maximal spanning forest. Since such proof is too big to specify and verify after every update, our definition allows such proof to be updated over input changes. (This is as opposed to specifying the densest subgraph from scratch every time as in \Cref{ex:subgraphDetect_inNP}.) Allowing this is crucial for most problems to be in $\dNP$, but create difficulties to prove $\dNP$-completeness. We remedy this by introducing rewards.

Note that if there is no reward in \Cref{def:intro:dNP}, then it is even easier to show that dynamic connectivity and other problems are in $\dNP$. Having an additional constraint about rewards potentially makes less problems verifiable.  Luckily, all natural problems that we are aware of that were verifiable without rewards remain verifiable with rewards.
Problems in $\dNP$ include decision/gap versions of $(1+\epsilon)$-approximate matching, planar nearest neighbor, and dynamic 3SUM; see \Cref{table:BPP-NP} for more. The concept of rewards (introduced while defining the class $\dNP$) will turn to be crucial when we attempt to show the existence of a complete problem in  $\dNP$. See~\ref{sec:contribution:np:completeness} and~\ref{sec:overview} for more details.

It is fairly easy to show that $\dP \subseteq \dNP$,  and we conjecture that $\dP \neq \dNP$.








\paragraph{Previous nondeterminism in the dynamic setting.}
The idea of nondeterministic dynamic algorithms is not completely new.
This was considered by Husfeldt and Rauhe \cite{HusfeldtR03} and their follow-ups \cite{PatrascuD06,PatrascuThesis,Yin10,LarsenNonDeterministic,WangY14}, and has played a key role in proving cell-probe lower bounds in some of these papers. 
As discussed in \cite{HusfeldtR03}, although it is straightforward to define a nondeterministic dynamic algorithm as the one that can make nondeterministic choices to process each update and query, there are different ways to handle how nondeterministic choices affect the states of algorithms which in turns affect how the algorithms handle future updates (called the ``side effects'' in \cite{HusfeldtR03}). For example, in \cite{HusfeldtR03} nondeterminism is allowed only for answering a query, which happens to occur only once at the very end. In \cite{PatrascuD06}, nondeterministic query answering may happen throughout, but an algorithm is allowed to write in the memory (thus change its state) only if all nondeterministic choices lead to the same memory state.

In this paper we define a different notion of nondeterminism and thus the class $\dNP$. It is more general than the previous definitions in that if a dynamic problem admits an efficient nondeterministic algorithm according to the previous definitions, it is in our $\dNP$.  
In a nutshell, the key differences are that (i) we allow nondeterministic steps while processing both updates and queries and (ii) different choices of nondeterminism  can affect the algorithm's states in different ways; however, we distinct different choices by giving them different rewards. 
These differences allow us to include more problems to our $\dNP$ (we do not know, for example, if dynamic connectivity admits nondeterministic algorithms according to previous definitions). 









\subsection{$\dNP$-Completeness}
\label{sec:contribution:np:completeness}

Here, we sketch the idea behind our $\dNP$-completeness and hardness results. 
We begin by introducing a  problem is called {\em dynamic narrow DNF evaluation problem} (in short, $\dDNF$), as follows. 


\begin{defn}[$\dDNF$; informally]\label{defn:intro:dnf}
Initially, we have to preprocess (i) an $m$-clause $n$-variable DNF formula\footnote{Recall that a DNF formula is in the form $C_{1}\vee\dots\vee C_{m}$, where each ``clause'' $C_i$ is a conjunction (AND) of literals.} where each clause contains $O(\polylog(m))$ literals, and (ii) an assignment of (boolean) values to the variables. Each update  changes the value of one variable. After each update, we have to answer whether the DNF formula is true or false. 
\end{defn}


It is fairly easy to see that $\dDNF \in \dNP$: After each update, if the DNF formula happens to be true, then the proof only needs to point towards one satisfied clause, and the verifier can quickly check if this clause is satisfied or not since it contains only $O(\polylog (m))$ literals. Surprisingly, it turns out that this is also a complete problem  in the classs $\dNP$.

\begin{theorem}[$\dNP$-completeness of $\dDNF$]\label{thm:intro:DNF}
The $\dDNF$ problem is $\dNP$-complete. This means that  $\dDNF\in \dNP$, and if $\dDNF\in \dP$, then $\dP=\dNP$.
\end{theorem}


To start with, recall the following intuition for proving NP-completeness in the static setting  (e.g. \cite[Section 6.1.2]{AroraBarak_book} for details): Since {\em Boolean circuits} can simulate polynomial-time Turing machine computation (i.e. $P \subseteq P \slash \mathsf{poly}$), we view the computation of the verifier $V$ for any problem $\Pi$ in NP as a circuit $C$. The input of $C$ is the proof that $V$ takes as an input. Then, determining whether there is an input (proof) that satisfies this circuit (known as  {\em CircuitSAT}) is NP-complete, since such information will allow the verifier to find a desired proof on its own.  Attempting to extend this intuition to the dynamic setting might encounter the following roadblocks.

\begin{enumerate}[label=(\roman*)]
\item Boolean circuits cannot efficiently simulate algorithms in the RAM model without losing a linear factor in running time.
Furthermore, an alternative such as circuits with ``indirect addressing'' gates seems useless, because this complex gate makes the model more complicated. 
This makes it more difficult to prove  $\dNP$-hardness.
\item Since the verifier has to work through several updates in the dynamic setting, the YES/NO output from the verifier alone is insufficient to indicate proofs that can be useful for {\em future} updates. For example, suppose that in \Cref{ex:intro:connectivity in NP}   the connectivity verifier is allowed to output only $x\in \{YES, NO\}$, and we get rid of the concept of a reward.  
Consider a scenario where 
an edge $e$ (which is part of $F$) gets deleted from $G$, and $G$ was disconnected even before this deletion. In this case, the verifier can indicate no difference between having $e'$ (i.e. finding a reconnecting edge) and $\bot$ (i.e. doing nothing) as a proof (because it has to output $x=0$ in both cases). Having $e'$ as a proof, however, is more useful for the future, since it  helps maintain a spanning forest.
\end{enumerate}

It so happens that we can solve (ii) if the verifier additionally outputs an integer $y$ as a reward. Asking more from the verifier  makes less problems verifiable (thus smaller $\dNP$).  Luckily, all natural problems we are aware of that were verifiable without rewards remain verifiable with rewards! 



To solve (i), we use the fact that in the cell-probe model a polylogarithmic-update-time algorithm can be modeled by a polylogarithmic-depth {\em decision assignment tree} \cite{Miltersen99cellprobe}, which naturally leads to a complete problem about a decision tree (we leave details here; see ~\ref{sec:overview} and~\Cref{sec:DT} for more).
It turns out that we can reduce from this problem to $\dDNF$ (\Cref{defn:intro:dnf}); the intuition being that each bit in the main memory corresponds to a boolean variable and each root-to-leaf path in the decision assignment tree can be thought of as a DNF clause. The only downside of this approach is that a  polylogarithmic-depth decision tree  has quasi-polynomial size. A straightforward reduction would cause quasi-polynomial space in the cell-probe model. By exploiting the special property of $\dDNF$ and the fact that the cell-probe model only counts the memory access, we can avoid this space blowup by ``hardwiring'' some space usage into the decision tree and reconstruct some memory when needed. 














The fact that the $\dDNF$ problem is $\dNP$-complete (almost) immediately implies  that many well-known dynamic problems are $\dNP$-hard. To explain why this is the case, we first recall the definition of the \emph{dynamic sparse orthogonal vector} ($\dOV$) problem.

\begin{defn}[$\dOV$]\label{def:OV}\label{main:def:OV}
Initially, we have to preprocess a collection of $m$ vectors  $V = \{ v_1, \ldots, v_{m} \}$ where each $v_j \in \{0,1\}^n$, and another vector $u \in \{0,1\}^n$.  It is guaranteed that each $v_j \in \{0,1\}^n$ has at most $O(\polylog (m))$ many nonzero entries. Each update flips the value of one entry in the vector $u$. After each update, we have to answer if there is a vector $v \in V$ that is orthogonal to $u$ (i.e., if $u^T v = 0$).
\end{defn}


\medskip
The key observation is that the $\dOV$ problem is equivalent to the $\dDNF$ problem, in the sense that $\dOV \in \dP$ iff $\dDNF \in \dP$. The proof is relatively straightforward (the vectors $v_j$ and the individual entries of $u$ respectively correspond to the clauses and the variables in $\dDNF$), and we defer it to~\ref{sec:DNF equiv proof}. In~\cite{AbboudW14}, Abboud and Williams show SETH-hardness for all
of the problems in \ref{main:table:NP hard}. In fact, they
actually show a reduction from $\dOV$ to these problems. Therefore, we immediately obtain the following result.
\begin{cor}
\label{main:cor:list rankNP hard}All problems in \ref{main:table:NP hard}
are $\dNP$-hard.
\end{cor}





\subsection{Dynamic Polynomial Hierarchy}




By introducing the notion of {\em oracles} (see~\ref{sec:model:dynamic}), it is not hard to extend the class $\dNP$ into {\em polynomial-hierarchy} for dynamic problems, denoted by $\dPH$. Roughly,  $\dPH$ is the union of classes $\dSigma_i$ and $\dPi_i$, where (i) $\dSigma_1= \dNP$, $\dPi_1=\dcoNP$,  and (ii) we say that a dynamic problem is in class $\dSigma_i$ (resp. $\dPi_i$) if we can show that it is in $\dNP$  (resp. $\dcoNP$) assuming that there are efficient dynamic algorithms for problems in $\Sigma_{i-1}$.   See~\ref{sec:PH} for more details.



\begin{example}[$k$- and (<$k$)-edge connectivity]\label{ex:intro:k-con in Pi2}
In the {\em dynamic $k$-edge connectivity} problem,  an $n$-node graph $G = (V, E)$ and a parameter $k = O(\polylog (n))$ is given at the time of preprocessing.  Each update is an edge insertion or deletion in $G$.  We want an algorithm to output YES if and only if $G$ has connectivity {\em at least $k$}, i.e. removing at most $k-1$ edges will {\em not} disconnect $G$. We claim that this problem is in $\dPi_2$. To avoid dealing with $\dcoNP$, we consider the complement of this problem called {\em dynamic (<$k$)-edge connectivity}, where $x=YES$ if and only if $G$ has connectivity less than $k$. We show that  (<$k$)-edge connectivity is in $\dSigma_2$. 
	

We already argued in \Cref{ex:intro:connectivity in NP} that dynamic connectivity is in $\dNP=\dSigma_1$. Assuming that there exists an efficient (i.e. polylogarithmic-update-time) algorithm  $\cal A$ for dynamic connectivity, we will show that  (<$k$)-edge connectivity is in $\dNP$. 
Consider the following verifier $\cal V$.  After every update in $G$, the verifier $\cal V$ reads a proof that is supposed to be a set $S \subseteq E$ of at most $k-1$ edges. $\cal V$ then  sends the update to $\cal A$ and also tells $\cal A$ to delete the edges in $S$ from $G$. If $\cal A$ says that $G$ is not connected at this point, then the verifier $\cal V$ outputs $x=YES$ with reward $y=1$; otherwise, the verifier $\cal V$  outputs $x=NO$ with reward $y=0$. Finally, $\cal V$ tells $\cal A$ to add the edges in $S$ back in $G$. 

Observe that if $G$ has connectivity less than $k$ and the verifier always receives a proof that maximizes the reward, then the proof will be a set of edges disconnecting the graph and $\cal V$ will answer YES. Otherwise, no proof can make $\cal V$ answer YES. Thus the dynamic (<$k$)-edge connectivity problem is in $\dNP$ if $\cal A$ exists. In other words, the problem is in $\dSigma_2$.
\end{example}


By arguments similar to the above example, we can show that other problems such as Chan's subset union and small diameter are in $\dPH$; see \Cref{table:PH} and~\ref{sec:PH:examples} for more. 


The theorem that plays an important role in our main conclusion (\Cref{thm:intro:results_summary}) is the following. 

\begin{theorem}\label{thm:intro:PH collapse}
If $\dP=\dNP$, then $\dPH=\dP$. 
\end{theorem}

To get an idea how to proof the above theorem, observe that if $\dP=\dNP$, then $\cal A$ in \Cref{ex:intro:k-con in Pi2} exists and thus dynamic (<$k$)-edge connectivity are in $\dSigma_1=\dNP$ by the argument in \Cref{ex:intro:connectivity in NP}; consequently, it is in $\dP$! This type of argument can be extended to all other problems in $\dPH$. 

\subsection{Other Results and Remarks}
\label{sec:contribution:other:results}


In previous subsections, we have stated two complexity results, namely $\dNP$-completeness/hardness and the collapse of $\dPH$ when $\dP=\dNP$. With right definitions in place, it is not a surprise that more can be proved. For example, we  obtain the following results:

\begin{enumerate}[noitemsep, label=(\Roman*)]
	\item \label{thm:intro:NPcoNP} If $\dNP\subseteq \dcoNP$, then $\dPH=\dNP\cap \dcoNP$.
	\item \label{thm:intro:MAcoMA} If $\dNP\subseteq  \dMA \cap \dcoMA$, then $\dPH \subseteq \dMA \cap \dcoMA$.
\end{enumerate}
Here, $\dcoNP$, $\dMA$, and $\dcoMA$ are analogues of complexity classes coNP, MA, and coMA.\footnote{Roughly, MA is similar to NP, except that the verifier can be randomized.} See \Cref{th:PH:collapse:next,lem:if NP in coMA} for more details.



While the coarse-grained complexity results in this paper are mostly resource-centric (in contrast to fine-grained complexity results that are usually centered around problems), we also show that this approach is helpful for understanding the complexity of specific problems as well, in the form of {\em non-reducibility}.
In particular, the following results  are  shown in \Cref{part:connectivity}:%


\begin{enumerate}[noitemsep]
	
	\item \label{item:intro:non_reducibility_1}Assuming $\dPH\neq \dNP\cap \dcoNP$, the two statements {\em cannot} hold at the same time.
	\begin{enumerate}[noitemsep,nolistsep]
		\item Connectivity is in $\dcoNP$. (This would be the case if it is in $\dP$.)
		\item One of the following problems is $\dNP$-hard: approximate minimum spanning forest (MSF), $d$-weight MSF, bipartiteness, 
		and $k$-edge connectivity. 
	\end{enumerate}
	
	\item $k$-edge connectivity is in $\dMA \cap \dcoMA$. Consequently,  assuming  $\dPH \not\subseteq \dMA \cap \dcoMA$, $k$-edge connectivity cannot be $\dNP$-hard. 
\end{enumerate}





Note that both ${\sf PH}\neq {\sf NP}\cap {\sf coNP}$ and ${\sf PH} \not\subseteq {\sf MA} \cap {\sf coMA}$ are widely believed in the static setting since refuting them means collapsing ${\sf PH}$. While we can show that $\dPH$ would also collapse if $\dPH= \dNP\cap \dcoNP$, it remains open whether this is the case for $\dPH \subseteq \dMA \cap \dcoMA$; in particular is $\dPH \supseteq\dMA \cap \dcoMA$?

When a problem $Y$ cannot be $\dNP$-hard, there is no efficient reduction from an $\dNP$-hard problem $X$ to  $Y$, where an efficient reduction is roughly to a way to handle each update for problem $X$ by making polylogarithmic number of updates to an algorithm for $Y$ (such reduction would make $Y$ an $\dNP$-hard problem). Consequently, this rules out efficient  reductions from dynamic OV, since it is $\dNP$-complete. As a result, this rules out a common way  to prove lower bounds based on SETH, since previously this was mostly done via reductions from dynamic OV \cite{AbboudW14}. (A lower bound for dynamic diameter is among a very few exception \cite{AbboudW14}.) 





\subsection{Relationship to Fine-Grained Complexity} 
\label{sec:contribution:fine:grained}

As noted earlier, it turns out that the dynamic OV problem is $\dNP$-complete. Since most previous reductions from SETH to dynamic problems (in the word RAM model) are in fact reductions from dynamic OV~\cite{AbboudW14}, and since any reduction in the word RAM model applies also in the (stronger) cell-probe model, we get many $\dNP$-hardness results for free. In contrast, our results above  imply that the following two statements are equivalent: (i)   ``problem $\Pi$ cannot be $\dNP$-hard'' and (ii) ``there is no {\em efficient} reduction from dynamic OV to $\Pi$'', where ``efficient reductions'' are reduction that only polynomially blow up the instance size (all reductions in \cite{AbboudW14} are efficient). In other words, we may not expect reductions from SETH that are similar to the previous ones for $k$-edge connectivity, bipartiteness, etc. 

Finally, we emphasize that the coarse-grained approach should be viewed as a complement of the fine-grained approach, as the above results exemplify. We do not expect to replace results from one approach by those from another. 


\subsection{Complexity classes for dynamic problems in the word RAM model}
\label{sec:contribution:word:RAM}

As an aside, we managed to define complexity classes and completeness results for dynamic problems in the word RAM model as well. 
We refer to $\dP$ and  $\dNP$ as $\dPram$ and $\dNPram$ in the word-RAM model. One caveat is that for technical reasons we need to allow for quasipolynomial preprocessing time and space while defining the complexity classes $\dPram$ and $\dNPram$. We discuss this in more details in \Cref{part:RAM}.









==> discussions.tex <==



\subsection{Discussions}\label{sec:discussions}







One challenge of this work is coming up with right definitions that allow us to compare inherit difficulties of many problems and at the same time reproduce traditional complexity results. For this reason, we also devote some space discussing our choices. 

\paragraph{Class $\dP$.}
To start with, we have to discuss what an analogue of class P should be for dynamic problems. In other words, what should ``efficient dynamic algorithms'' mean? Recall that the terms efficient algorithms and class P in the static setting refer to deterministic algorithms with running time polynomial in the input size. 
Since the main inputs of dynamic algorithms are updates\footnote{Note again that dynamic algorithms usually also has queries, but they can formally defined as updates so we will ignore the queries here.}, a natural definition of efficient dynamic algorithms is algorithms with update time polynomial in the {\em update size}, the number of bits to describe the updates. 

This definition in fact conforms with algorithms desired for many dynamic problems. For example, an update for most dynamic graph problems is an edge insertion or deletion -- a polylogarithmic-size update -- and it is typically desirable that algorithms for these problems have polylogarithmic update time. Problems mentioned in \Cref{thm:intro:results_summary} are also of this nature, and well known data structures, such as priority queues, disjoint-set data structures, dynamic range searching and link/cut trees, are also efficient in this sense. In fact, since most natural dynamic problems have polylogarithmic update size, we will focus on this case in this paper to avoid cumbersome notations. We note how our results translate to larger update size later.

Typically it is also desirable that dynamic algorithms have polynomial preprocessing time. As will be more clear later, in order to prove our $\dNP$-hardness results, it is crucial to {\em relax} the preprocessing time to quasi-polynomial, and consequently quasi-polynomial space. 
We discuss this relaxation more below.
To conclude:
\begin{defn}[$\dP$; brief]\label{def:intro:dP}
The class $\dP$ contains any dynamic problem with polylogarithmic update size that admits an algorithm with polylogarithmic update time and quasi-polynomial preprocessing time and space.
\end{defn}
Our examples of problems in $\dP$ are in \Cref{table:P}. 
Note that we have not defined what dynamic problems are formally. Such definition is needed to define the class $\dP$ formally and can be found in XXX. 






\paragraph{Class $\dNP$:}
Recall that in the static setting NP is the set of problems with efficiently verifiable proofs or, equivalently, solvable in polynomial time by a nondeterministic algorithm. It is natural to define $\dNP$ the same way; i.e. an algorithm can make a nondeterministic choice to handle each update (or equivalently a verifier has to verify in polylogarithmic time  a polylogarithmic-size proof provided by a powerful prover).
This idea is in fact not completely new. The notion of {\em nondeterministic queries} was considered by Husfeldt and Rauhe \cite{HusfeldtR03} and their follow-ups \cite{PatrascuD06,PatrascuThesis,Yin10,LarsenNonDeterministic,WangY14}, and has played a key role in proving cell-probe lower bounds in some of these papers. 



The above straightforward extension however has an important issue to be addressed: different nondeterministic choices lead to different states of an algorithm, which might affect how the algorithm handles future updates. This issue was, for example, handled in \cite{PatrascuD06} by allowing algorithms to write in the memory only if all nondeterministic choices lead to the same memory state and limiting the nondeterministic choices to only answering queries.  This option is too limited for us to capture natural dynamic problems in $\dNP$ and $\dPH$. In this paper we define a different notion of nondeterminism and thus the class $\dNP$. It is more general than the previous definition in that if a dynamic problem admits an efficient nondeterministic algorithm according to the previous definition, it is in our $\dNP$. 

Our notion of nondeterminism is captured by the proof verification notion where verifier does not only output  YES/NO, but also {\em rewards} after reading each proof.

The prover is then supposed to maximize this reward at every step. More precisely:
\begin{defn}[$\dNP$; brief]\label{def:intro:dNP}
We say that a dynamic problem $X$ with polylogarithmic update size is in $\dNP$ if there is a verifier that (i) takes quasi-polynomial preprocessing time, (ii) after every update takes the update and a polylogarithmic-size proof from the prover as an input, and (iii) after each update outputs in polylogarithmic time a pair $(x, y)$, where $x\in \{YES,NO\}$ and $y$ is an integer (representing a reward) with the following properties.
	\begin{itemize}[noitemsep]
		\item If the current input instance is a YES-instance, and if the prover always provides a proof that maximizes the reward at every step then the verifier outputs $X=YES$.
		\item If the current input instance is a NO-instance, then the verifier outputs $X=NO$  regardless of what the proofs are so far. \qedhere
	\end{itemize}
\end{defn} 
 
 

 

==> hardness_sayan.tex <==

\section{$\protect\drankNP$-complete Problems}


\subsection{Notations needed.}
\begin{enumerate}
\item The meta-graph $\G_{n}=(\U_{n},\E_{n})$. 
\item While defining a decision tree: 

\begin{itemize}
\item $T(\mem)$: output of the decision tree while operating on the memory
$\mem$. 
\end{itemize}
\item While defining an algorithm $\A_{n}$: 

\begin{itemize}
\item Inputs to an algorithm $\A_{n}$: $\inp_{\A_{n}}(0),\ldots,\inp_{\A_{n}}(i),\ldots$. 
\item $\init_{\A_{n}}:\{0,1\}^{*}\rightarrow\{0,1\}$. Once it gets input
$\inp_{0}$ at step $0$, it sets $\mem_{\A_{n}}=\init_{\A_{n}}(\inp_{\A_{n}}(0))$. 
\item $T_{\A_{n}}$: decision tree followed by the algorithm. 
\item $\mem_{\A_{n}}$, 
\item $\mem_{\A_{n}}$ is partitioned into $\mem_{\A_{n}}^{\work}$, $\mem_{\A_{n}}^{\inp}$
and $\mem_{\A_{n}}^{\out}$. 
\end{itemize}
\item While defining an oracle: 

\begin{itemize}
\item $\mem_{\A_{n}}^{\work}$ is partitioned into $\mem_{\A_{n}}^{0},\mem_{\A_{n}}^{1},\ldots,\mem_{\A_{n}}^{m}$. 
\item For each $j\in[1,m]$, $\mem_{\A_{n}}^{j}=\mem_{O_{n_{j}}}$. That
is, $\mem_{\A_{n}}^{j}$ is the memory for the oracle $O_{n_{j}}$. 
\end{itemize}
\item While defining the class $\drankNP$: 

\begin{itemize}
\item Verifier $\V_{n}$. There exists a polynomial $p$ such that each
proof-update $\pi\in\{0,1\}^{p(\lambda_{n})}$. The input memory $\mem_{\A_{n}}^{\inp}$
is partitioned into two halves for a verifier: $\mem_{\V_{n}}^{\inst}$
and $\mem_{\V_{n}}^{\prf}$. 
\item $\prec_{\P_{n}}^{0}$ and $\prec_{\P_{n}}$. 
\end{itemize}
\end{enumerate}

\subsection{First Decision Tree Evaluation (FTDE) problem}

We start by giving an intuitive and (slightly) informal definition
of the FTDE problem. In the static setting, the problem is denoted
by $\P'$. An instance $I\in\P'$ of this problem consists of a collection
of decision trees $\T_{I}$ arranged according to a total ordering
$\prec_{I}$, and a finite array of bits $\mem_{I}$. Each decision
tree $T\in\T_{I}$ operates on the same memory $\mem_{I}$. The answer
$\P'(I)$ is equal to the index of the first decision tree $T\in\T_{I}$
according to the total ordering $\prec_{I}$ such that $T(\mem_{I})\neq\bot$,\footnote{In other words, $T$ produces a valid output when applied to the memory
configuration $\mem_{I}$.} provided such an index exists. Otherwise, if $T(\mem_{I})=\bot$
for all $T\in\T_{I}$, then $\P'(I)=\bot$. In the dynamic setting,
the instance $I$ keeps changing via a sequence of updates where each
update changes the content of exactly one bit in the memory $\mem_{I}$,
and we have to keep track of the answer $\P'(I)$ at the current instance
$I$. Below, we give a formal definition.

The FTDE problem is denoted by $\P'$ in the static setting. An instance
$I\in\P'$ of this problem is encoded as a tuple $(\mem_{I},\Pi_{I},\prec_{I},\T_{I})$,
where $\mem_{I}$ denotes a finite array of bits, $\Pi_{I}\subseteq\{0,1\}^{*}$
denotes a collection of bit-strings, $\prec_{I}$ denotes a total
ordering over $\Pi_{I}$, and $\T_{I}=\{T_{\pi}:\pi\in\Pi_{I}\}$
denotes a collection of decision trees. Each decision tree $T_{\pi}\in\T_{I}$
operates on the same memory $\mem_{I}$. Let $\T_{I}^{valid}=\{T_{\pi}\in\T_{I}:T_{\pi}(\mem_{I})\neq\bot\}$
denote the set of decision trees $T_{\pi}\in\T_{I}$ that produce
valid outputs when applied to the memory configuration $\mem_{I}$.
The answer $\P'(I)$ is defined as follows. 
\begin{itemize}
\item If $\T_{I}^{valid}=\emptyset$, then $\P'(I)=\bot$. Otherwise, if
$\T_{I}^{valid}\neq\emptyset$, then $\P'(I)=\pi'$, where $\pi'$
is the first bit-string $\pi\in\Pi_{I}$ according to the total order
$\prec_{I}$ such that $T_{\pi}\in\T_{I}^{valid}$. 
\end{itemize}
For each integer $n\geq1$, let $\P'_{n}$ denote the $n$-slice of
the FTDE problem, which consists of all FTDE instances $I\in\P'$
that are encoded using $n$ bits. To define the FTDE problem in the
dynamic setting, for every integer $n\geq1$ we have to impose a graph
structure $\G'_{n}=(\U'_{n},\E'_{n})$ on $\P'_{n}$. We now define
the meta-graph $\G'_{n}=(\U'_{n},\E'_{n})$ where $\U'_{n}=\{0,1\}^{n}$.
For any two instances $I,I'\in\P'_{n}$, there is a directed meta-edge
$(I,I')\in\E'_{n}$ iff $\Pi_{I}=\Pi_{I'}$, $\prec_{I}=\prec_{I'}$,
$\T_{I}=\T_{I'}$, and $\mem_{I}$ and $\mem_{I'}$ differ in exactly
one bit. Hence, the standard encoding of an instance-update $(I,I')\in\E'_{n}$
can be specified using at most $\log n$ bits, and we get the following
upper bound on the instance-update size of this problem: $\lambda'_{n}\leq\log n$.
We denote the dynamic FDTE problem by $(\P',\G')$, and the $n$-slice
of this problem by $(\P'_{n},\G'_{n})$. The main result of this section
is summarized in the theorem below.
\begin{thm}
\label{th:np-hardness} For every problem $(\P,\G)\in\drankNP$, there
is a Cook reduction from $(\P,\G)$ to $(\P',\G')$. 
\end{thm}
We devote the rest of this section to the Proof of Theorem~\ref{th:np-hardness}.
Towards this end, fix an integer $n\geq1$, and consider the $n$-slice
$(\P_{n},\G_{n})$ of the problem $(\P,\G)\in\drankNP$. Let $\V_{n}$
be a verifier for $(\P_{n},\G_{n})$ which satisfy~\ref{def:rankNP}.
Consider an integer $b=b(n)$, whose value will be fixed later on.
We will describe an algorithm $\A_{n}$ for $(\P_{n},\G_{n})$ which
has access to an oracle for $(\P'_{b},\G'_{b})$ and has an update
time of $O(\text{poly}(\lambda_{n}))$. This will imply the theorem.

\medskip{}
To see how the algorithm $\A_{n}$ works, consider any directed path
$(I_{0},\ldots,I_{k})$ in the meta-graph $\G_{n}=(\V_{n},\E_{n})$,
and let $\inp_{\A_{n}}(0\rightarrow k)=\inp_{\A_{n}}(0),\ldots,\inp_{\A_{n}}(k)$
be the input sequence corresponding to this path. We have $\inp_{\A_{n}}(0)=I_{0}$
and $\inp_{\A_{n}}(t)=u(I_{t-1},I_{t})$ for each $t\in\{1,\ldots,k\}$.
We will describe how the algorithm $\A_{n}$ handles this input sequence.
Specifically, consider the following process. 
\begin{itemize}
\item For $t=0$ to $k$: 

\begin{itemize}
\item The algorithm $\A_{n}$ receives the input $\inp_{\A_{n}}(t)$ at
step $t$, handles this input {\em without looking ahead into the
future}, and produces an output $\A_{n}(\inp_{\A_{n}}(0\rightarrow t))$. 
\end{itemize}
\end{itemize}
We will ensure that $\A_{n}(\inp_{\A_{n}}(0\rightarrow t))=\P_{n}(I_{t})$
for all $t\in\{0,\ldots,k\}$. In words, this means that the algorithm
$\A_{n}$ always produces the correct output for $(\P_{n},\G_{n})$
while handling the input sequence $\inp_{\A_{n}}(0\rightarrow k)$.
We will also ensure that the update time of $\A_{n}$ is at most $O(\text{poly}(\lambda_{n}))$.
Our algorithm $\A_{n}$ will use the verifier $\V_{n}$ as a subroutine
and will have access to an oracle for $(\P'_{b},\G'_{b})$. In order
to explain how this works, we have to introduce the following notations.

\medskip{}
The verifier handles an update operation according to the decision
tree $T_{\V_{n}}$ which operates on the memory $\mem_{\V_{n}}$.
Further, recall that the input memory $\mem_{\V_{n}}^{\inp}$ of the
verifier is partitioned into two parts: $\mem_{\V_{n}}^{\inst}$ and
$\mem_{\V_{n}}^{\prf}$. Let $\mem_{\V_{n}}^{*}=\mem_{\V_{n}}\setminus\mem_{\V_{n}}^{\prf}$
be an array denoting all the bits in the memory of the verifier, except
the ones containing the proof-update $\pi$. For each $\pi\in\{0,1\}^{p(\lambda_{n})}$,
let $T_{\V_{n}}^{(\pi)}$ be a decision-tree that mimics the behavior
of the decision tree $T_{\V_{n}}$ when $\mem_{\V_{n}}^{\prf}=\pi$.
Specifically, the decision tree $T_{\V_{n}}^{(\pi)}$ operates on
the memory $\mem_{\V_{n}}^{*}$ and satisfies the following property:
For all configurations of $\mem_{\V_{n}}$ with $\mem_{\V_{n}}^{\prf}=\pi$,
we have $T_{\V_{n}}^{(\pi)}\left(\mem_{\V_{n}}^{*}\right)=T_{\V_{n}}(\mem_{\V_{n}})$.
Define the collection of decision trees $\T_{\V_{n}}=\left\{ T_{\V_{n}}^{(\pi)}:\pi\in\{0,1\}^{p(\lambda_{n})}\right\} $
and let $\Pi_{\V_{n}}=\{0,1\}^{p(\lambda_{n})}$. Define $b=b(n)$
so that it takes $b$ bits to encode an instance $I'=(\mem_{\V_{n}}^{*},\Pi_{\V_{n}},\prec_{\P_{n}},\T_{\V_{n}})\in\P'$.
The algorithm $\A_{n}$ maintains the instance $I'=(\mem_{\V_{n}}^{*},\Pi_{\V_{n}},\prec_{\P_{n}},\T_{\V_{n}})$,
which keeps changing dynamically because $\mem_{\V}^{*}$ keeps changing
with time. The oracle for $(\P'_{b},\G'_{b})$ maintains the answer
$\P'_{b}(I')$.

\medskip{}
We now describe how the algorithm $\A_{n}$ works, using induction
on step $t\in\{0,\ldots,k\}$.


\subsubsection{Base Case: Handling the input operation $\protect\inp_{\protect\A_{n}}(0)$
at step $t=0$}

\label{sec:base}

At step $t=0$, the algorithm $\A_{n}$ receives the input $\inp_{\A_{n}}(0)=I_{0}$.
Let $\pi_{0}\in\{0,1\}^{p(n)}$ be the first (and hence unique) proof
according to the total order $\prec_{\P_{n}}^{0}$ such that the verifier
$\V_{n}$ produces a valid output when asked to handle the preprocessing
operation with input $(I_{0},\pi_{0})$. Define $\inp_{\V_{n}}(0)=(I_{0},\pi_{0})$.
By~\ref{def:rankNP}, such a proof $\pi_{0}$ always exists, and
$\inp_{\V_{n}}(0\rightarrow0)$ is a guaranteed input sequence for
the verifier $\V_{n}$. The algorithm $\A_{n}$ uses the verifier
$\V_{n}$ as a subroutine. Specifically, it sets $\mem_{\V_{n}}\leftarrow\init_{\V_{n}}(\inp_{\V_{n}}(0))$,
and outputs $\A(I_{0})=\V_{n}(\inp_{\V_{n}}(0\rightarrow0))=\P_{n}(I_{0})$.
Since $\inp_{\V_{n}}(0\rightarrow0)$ is a guaranteed input sequence
for the verifier, we get $\A(I_{0})=\P_{n}(I_{0})$. In words, the
algorithm $\A_{n}$ produces the correct output while handling the
preprocessing operation $\inp_{\A_{n}}(0)$. Finally, the algorithm
$\A_{n}$ initializes the instance $I'\in\P'_{b}$ by setting $I'=(\mem_{\V_{n}}^{*}(0),\Pi_{\V_{n}},\prec_{\P_{n}},\T_{\V_{n}})$,
where $\mem_{\V_{n}}^{*}(0)$ is the configuration of $\mem_{\V_{n}}^{*}$
after the verifier handles the input sequence $\inp_{\V_{n}}(0\rightarrow0)$.


\subsubsection{Inductive Case: Handling the input operation $\protect\inp_{\protect\A_{n}}(t)$
at step $t\in\{1,\ldots,k\}$}

\label{sec:induction} By induction hypothesis, assume that we are
at the situation outlined below.
\begin{prop}
\label{prop:induction} Till this point, the algorithm $\A_{n}$ has
handled the input sequence $\inp_{\A_{n}}(0\rightarrow t-1)$ and
the verifier $\V_{n}$ (used as a subroutine by $\A_{n}$) has handled
the guaranteed input sequence $\inp_{\V_{n}}(0\rightarrow t-1)$,
where $\inp_{\V_{n}}(0)=(I_{0},\pi_{0})$ and $\inp_{\V_{n}}(j)=\left(u(I_{j-1},I_{j}),\pi_{j}\right)$
for all $j\in\{1,\ldots,t-1\}$. Further, at this point, the instance
$I'\in\P'_{b}$ is defined as $I'=(\mem_{\V_{n}}^{*}(t-1),\Pi_{\V_{n}},\prec_{\P_{n}},\T_{\V_{n}})$,
where $\mem_{\V_{n}}^{*}(t-1)$ is the configuration of $\mem_{\V_{n}}^{*}$
after the verifier handles the guaranteed input sequence $\inp_{\V_{n}}(0\rightarrow t-1)$. 
\end{prop}
Now, upon receiving the input $\inp_{\A_{n}}(t)=u(I_{t-1},I_{t})$,
the algorithm $\A_{n}$ works as follows. It finds a specific proof-update
$\pi_{t}\in\{0,1\}^{p(\lambda_{n})}$ and sets $\inp_{\V_{n}}(t)=\left(u(I_{t-1},I_{t}),\pi_{t}\right)$.
The proof-update $\pi_{t}$ is chosen in such a way which ensures
that $\inp_{\V_{n}}(0\rightarrow t)$ is a guaranteed input sequence
for the verifier $\V_{n}$. By~\ref{prop:induction} and~\ref{def:rankNP},
such a proof-update $\pi_{t}$ must exist. The algorithm $\A_{n}$
then asks the verifier $\V_{n}$ to handle the input operation $\inp_{\V_{n}}(t)$.
When the verifier returns, the algorithm $\A_{n}$ outputs the answer
$\A_{n}(\inp_{\A_{n}}(0\rightarrow t))=\V_{n}(\inp_{\V_{n}}(0\rightarrow t))$.
Since $\inp_{\V_{n}}(0\rightarrow t)$ is a guaranteed input sequence
for the verifier $\V_{n}$, we have $\A_{n}(\inp_{\A_{n}}(0\rightarrow t))=\P_{n}(I_{t})$.
Thus, the algorithm $\A_{n}$ produces the correct output while handling
the update operation $\inp_{\A_{n}}(t)$.

\medskip{}
\textbf{Finding the proof-update $\pi_{t}$ using the oracle for $(\P'_{b},\G'_{b})$.}
In order to find the proof-update $\pi_{t}$, the algorithm $\A_{n}$
crucially uses its access to the oracle for $(\P'_{b},\G'_{b})$.
To see how this works, let us get back to the situation outlined in~\ref{prop:induction},
and suppose that the algorithm $\A_{n}$ is now asked to handle the
input operation $\inp_{\A_{n}}(t)$. By~\ref{def:rankNP}, the proof-update
$\pi_{t}$ the algorithm $\A_{n}$ is looking for is the first proof-update
$\pi\in\Pi_{\V_{n}}=\{0,1\}^{p(\lambda_{n})}$ according to the total
order $\prec_{\P_{n}}$ such that the verifier $\V_{n}$ would produce
a valid output if it is asked to handle the update operation $\inp_{\V_{n}}(t)=\left(u(I_{t-1},I_{t}),\pi\right)$
at this stage. Equivalently, the proof-update $\pi_{t}$ is the first
proof-update $\pi\in\Pi_{\P_{n}}$ according to the total order $\prec_{\P_{n}}$
such that $T_{\V_{n}}(\mem_{\V_{n}})\neq\bot$ when $\mem_{\V_{n}}^{\prf}=\pi$.
This, in turn, means that $\pi_{t}$ is the first proof-update $\pi\in\Pi_{\V_{n}}$
as per the total order $\prec_{\P_{n}}$ such that $T_{\V_{n}}^{(\pi)}(\mem_{\V_{n}}^{*})\neq\bot$.
Thus, we infer that $\pi_{t}=\P'_{b}(I')$ where $I'=(\mem_{\V_{n}}^{*},\Pi_{\V_{n}},\prec_{\P_{n}},\T_{\V_{n}})$.
In other words, the algorithm $\A_{n}$ can figure out the proof-update
$\pi_{t}$ by querying the oracle for $(\P'_{b},\G'_{b})$. Specifically,
the algorithm $\A_{n}$ uses the oracle for $(\P'_{b},\G'_{b})$ as
follows. 
\begin{enumerate}
\item After receiving the input $\inp_{\A_{n}}(t)=u(I_{t-1},I_{t})$, the
algorithm $\A_{n}$ sets $\mem_{\V_{n}}^{\inst}=u(I_{t-1},I_{t})$.
This changes the instance $I'$. However, since the instance-update
$u(I_{t-1},I_{t})$ is encoded using at most $\lambda_{n}$ bits,
the algorithm can find the answer $\P'_{b}(I')$ to the new instance
$I'$ by making at most $\lambda_{n}$ many updates to the oracle
for $(\P'_{b},\G'_{b})$. Note that $\pi_{t}$ is equal to the answer
$\P'_{b}(I')$ to the new instance $I'$. 
\item After obtaining $\pi_{t}$, the algorithm instructs the verifier to
handle the update operation $\inp_{\V_{n}}(t)=\left(u(I_{t-1},I_{t}),\pi_{t}\right)$.
The algorithm outputs $\A_{n}(\inp_{\A_{n}}(0\rightarrow t))=\V_{n}(\inp_{\V_{n}}(0\rightarrow t))$.
Note that the update operation $\inp_{\V_{n}}(t)$ changes at most
$\text{poly}(\lambda_{n})$ bits in the memory $\mem_{\V_{n}^{*}}$,
because the verifier had $O(\text{poly}(\lambda_{n}))$ update time.
The algorithm then goes ahead and changes the instance $I'$ accordingly,
by making at most $O(\text{poly}(\lambda_{n}))$ many updates to the
oracle for $(\P'_{b},\G'_{b})$. 
\end{enumerate}

\subsection{First DNF Evaluation (FDNF) problem}

\noindent Intuitively, the dynamic FDNF problem can be defined as
follows. We are given a set of variables, a sequence of clauses defined
over these variables where each clause is a conjunction of literals,
and an assignment of values to the variables. An {\em instance-update}
consists of changing the value of exactly one variable. A dynamic
algorithm for this problem has to maintain the first clause in the
sequence (if any) that is satisfied under the current assignment of
values to the variables. Below, we give a more formal description
of this problem according to the notations from~\ref{sec:problem}.

\medskip{}
 In the static setting, an instance of the FDNF problem is given by
a triple $(\X,\C,\phi)$ such that: 
\begin{enumerate}
\item $\X$ is a set of $t_{v}$ boolean variables $\{x_{1},\ldots,x_{t_{v}}\}$. 
\item $\C$ is a sequence of $t_{c}$ clauses $C_{1},\ldots,C_{t_{c}}$
defined over $\X$, where each $C_{j}$ is a conjunction (AND) of
at most $t_{s}$ literals (variables or their negations). 
\item $\phi:\X\rightarrow\{0,1\}$ is an assignment of values to each variable
in $\X$. 
\end{enumerate}
\noindent Let $N=N(t_{v},t_{c},t_{s})$ denote the number of bits
needed to represent an instance of this problem. Note that $N=\text{poly}(t_{v},t_{c},t_{s})$.
Given any instance $I\in\{0,1\}^{N}$ of this problem, we use the
symbols $\X_{I},\C_{I}$ and $\phi_{I}$ to respectively denote the
set of variables, sequence of clauses and assignment of values to
the variables in $I$. The FDNF problem is given by a function $\P'_{N}:\{0,1\}^{N}\rightarrow\{0,1\}^{*}$
which is defined as follows. Consider any instance $I\in\{0,1\}^{N}$.
If no clause in $\C_{I}$ is satisfied under the assignment $\phi_{I}$,
then we have $\P'_{N}(I)=0$. Otherwise, the answer $\P'_{N}(I)$
is equal to the binary representation of the smallest index $t\in\{1,\ldots,t_{c}\}$
such that the clause $C_{t}$ in $\C_{I}$ is satisfied under the
assignment $\phi_{I}$.

In the dynamic setting, the FDNF problem imposes a directed meta-graph
$\G'_{N}=(\V'_{N},\E'_{N})$ over the set of all instances $\V'_{N}=\{0,1\}^{N}$.
There exists a meta-edge $(I,I')\in\E'_{N}$ between two meta-nodes
$I,I'\in\V'_{N}$ iff $\X_{I}=\X_{I'}$, $\C_{I}=\C_{I'}$ and the
assignments $\phi_{I},\phi_{I'}$ differ only in the value of exactly
one variable. It follows that the standard encoding $u(I,I')$ of
an instance-update $(I,I')\in\E'_{N}$ requires $O(\log N)$ bits.
So the dynamic problem $(\P'_{N},\G'_{N})$ has an instance-update
size of $\lambda'_{N}=O(\log N)$.

There exists a standard mapping between decision trees and DNF instances.
Basically, consider any decision tree $T$ that operates on memory
$\mem$. We can treat each bit in the memory as a variable, and each
root to leaf path in $T$ as a conjunctive clause formed out of the
memory variables corresponding to this path. This, along with~\ref{th:np-hardness}
leads to the following corollary.
\begin{cor}
\label{cor:np-hard} The dynamic FDNF problem is $\drankNP$-hard. 
\end{cor}




==> hypothesis.tex <==

\section{Hardness of OMv}
\begin{conjecture}
For any constant $\epsilon>0$, there is a constant $k$ such that
there is no algorithm for independent set query on any $n$-node $k$-uniform
hypergraph with $O(n^{k(1-\epsilon)})$ query time. \end{conjecture}


****What about when $k=\polylog(n)$?******

\begin{lem}
Suppose there is an algorithm for independent set query on an $N$-node
graph $G$ with query time $O(N^{2(1-\epsilon)})$ for some constant
$\epsilon>0$. Then, for any $n$ and $k$, there is an algorithm
for independent set query on an $n$-node $2k$-uniform hypergraph
$H$ with query time $O(N^{2(1-\epsilon)})=O(n^{2k(1-\epsilon)})$
where $N=\binom{n}{k}$.\end{lem}
\begin{proof}
Given an $n$-node $2k$-uniform hypergraph $H=(V_{H},E_{H})$, we
create a graph $G=(V_{G},E_{G})$ as follows. For each set $S\subseteq V_{H}$
where $|S|=k$, there is a node $v_{S}\in V_{G}$. For each hyperedge
$e\in E_{H}$ and for each partition of edge $e=S_{1}\cup S_{2}$
where $|S_{1}|=|S_{2}|=k$, we create an edge $(v_{S_{1}},v_{S_{2}})\in E_{G}$. 

Given a query $S_{H}\subseteq V_{H}$, we will create a set $T_{G}=\{v_{S}\mid S\subseteq S_{H}\}$.
If there is an edge $e_{H}\in E_{H}$ where $e_{H}\subseteq S_{H}$,
then there is an edge of $E$ inside $T_{G}$. For another direct,
suppose there is an edge $e_{G}\in E_{G}$ inside $T_{G}$. Let $e_{G}=(v_{S_{1}},v_{S_{2}})$.
As $v_{S_{1}},v_{S_{2}}\in T_{G}$, we have $S_{1},S_{2}\subseteq S_{H}$.
Moreover, there is an edge $e_{H}=S_{1}\cup S_{2}$ where $e_{H}\subseteq S_{H}$.
So $T_{G}$ is independent iff $S_{H}$ is independent.
\end{proof}
So we obtain a conjecture that implies the hardness OMv.


==> introduction.tex <==
\section{Introduction}\label{sec:intro}




In  a {\em dynamic problem}, we first get an input instance for {\em preprocessing}, and subsequently we have to handle a sequence of {\em updates} to the input.
For example, in the graph connectivity problem \cite{HenzingerK99,KapronKM13}, an $n$-node graph $G$ is given to an algorithm to preprocess. 
Then the algorithm has to answer whether $G$ is connected or not after each edge insertion and deletion to $G$. (Some dynamic problems also consider {\em queries}.\footnote{For example, in the connectivity problem an algorithm may be queried whether two nodes are in the same connected component or not.} Since queries can be phrased as input updates themselves, we will focus only on updates in this paper;  see \Cref{sec:model} for formal definitions and examples.) 
Algorithms that handle dynamic problems are known as {\em dynamic algorithms}. 
The {\em preprocessing time} of a dynamic algorithm is the time it takes to handle the initial input, whereas the worst-case {\em update time} of a dynamic algorithm is the {\em maximum} time it takes to handle any update.
Although dynamic algorithms are also analyzed in terms of their {\em amortized update times}, %
we emphasize that the results in this paper deal only with worst-case update times.
A holy grail for many dynamic problems -- especially those concering dynamic {\em graphs}  under edge deletions and insertions -- is to design algorithms with
{\em polylogarithmic update times}. From this perspective, the computational status of many classical dynamic problems still remain widely open. 




\paragraph{Example: Family of Connectivity Problems.} 
A famous example of a widely open question is for the family of connectivity problems:
(i) The problem of maintaining whether the input dynamic graph is connected (the dynamic {\em  connectivity} problem) admits a {\em randomized} algorithm with polylogarithmic worst-case update time. It is an active, unsettled line of research to determine whether it admits  deterministic polylogarithmic worst-case update time (e.g.~\cite{Frederickson85,EppsteinGIN92,HenzingerK99,HolmLT98,Thorup00,PatrascuD06,KapronKM13,Wulff-Nilsen17,NanongkaiS17,NanongkaiSW17}). 
(ii) The problem of maintaining whether the input dynamic graph can be disconnected by deleting an edge (the dynamic {\em $2$-edge connectivity} problem) admits polylogarithmic amortized update time \cite{HolmLT98,HolmRT18}, but its worst-case update time (even with randomization) remains polynomial \cite{Thorup01}. (iii) For dynamic $k$-edge connectivity with $k\geq 3$, the best update time -- amortization and randomization allowed -- suddenly jumps to $\tilde O(\sqrt{n})$ where 

$\tilde O$ hides polylogarithmic terms. Indeed, it is a major open problem to maintain a $(1+\epsilon)$-approximation to the value of global minimum cut in a dynamic graph in polylogarithmic update time~\cite{Thorup01}. Doing so for $k$-edge connectivity with $k=O(\log n)$ is already sufficient to solve the general case.

Other dynamic  problems that are not known to admit polylogarithmic update times include approximate matching, shortest paths, diameter, max-flow, etc.~\cite{Thorup01,Sankowski07}.

Thus, it is natural to ask: {\em can one argue that these problems do not admit efficient dynamic algorithms?}

A traditionally popular approach to  answer the question above is to use information-theoretic arguments in the {\em bit-probe/cell-probe model}. 
In this model of computation,  all the operations are free {\em except} memory accesses.\footnote{In more details, the bit-probe model concerns the number of bits accessed, while the cell-probe model concerns the number of accessed cells, typically of logarithmic size.} Lower bounds via this approach are usually {\em unconditional}, meaning that it does not rely on any assumption. 
Unfortunately, this approach could only give small lower bounds so far; and getting a super-polylogarithmic lower bound for {\em any} natural dynamic problem is an outstanding open question is this area~\cite{Larsen17boolean}. 

More recent advances towards answering this question arose from a new area called {\em fine-grained complexity}. While traditional complexity theory (henceforth we refer to it as  {\em coarse-grained complexity}) focuses on classifying problems based on resources and relating together resulting classes (e.g. P and NP), fine-grained complexity gives us {\em conditional} lower bounds in the word RAM model based on various assumptions about specific problems. For example, assumptions that are particularly useful for dynamic algorithms are the Strong Exponential Time Hyposis (SETH), which concerns the running time for solving SAT,  and the Online Matrix-Vector Multiplication Conjecture (OMv), which concerns the running time of certain matrix multiplication methods (more at, e.g., \cite{Patrascu10,AbboudW14,OMV}). 
In sharp contrast to cell-probe lower bounds, these assumptions often lead to polynomial lower bounds in the word RAM model, many of which are tight. 








While the  fine-grained complexity approach has led to many exciting lower bound results, there are a number of traditional results in the static setting that seem to have {\em no} analogues in the dynamic setting. 
For example, one reason that makes the $P\neq NP$ assumption so central in the static setting is that proving and disproving it will both lead to stunning consequences:  If the assumption is false then hundreds of problems in NP and bigger complexity classes like the polynomial hierarchy (PH) admit efficient algorithms; otherwise the situation will be the opposite.\footnote{For further consequences see, e.g., \cite{Aaronson17,Cook2006p,Cook03} and references therein.}
 
In contrast, we do not see any immediate consequence to dynamic algorithms if someone falsified SETH, OMv, or any other assumptions.\footnote{An indirect consequence would be that some barriers were broken and we might hope to get better upper bounds. This is however different from when P=NP where many hard problems would immediately admit efficient algorithms. Note that some consequences of falsifying SETH have been shown recently (e.g. \cite{AbboudBDN18,Williams13,GaoIKW17,CyganDLMNOPSW16,SanthanamS12,JahanjouMV15,DantsinW13}); however, we are not aware of any consequence to dynamic algorithms. It might also be interesting to note that Williams~\cite{Williams18-likelihood} estimates the likelihood of SETH to be only 25\%.}
As another example, comparing complexity classes allows us to speculate on various situations such as non-reducibility (e.g. \cite{AharonovR05,KlivansM02,Condon92}), the existence of NP-intermediate problems \cite{Ladner75} and the derandomization possibilities (e.g. \cite{ImpagliazzoW97}). (See more in \Cref{sec:open}.)
We cannot anticipate results like these in the dynamic setting without the coarse-grained approach, i.e. by considering analogues of P, NP, BPP and other complexity classes that are defined based on computational resources. 







\paragraph{Our Main Contributions.} We initiate a systematic study of coarse-grained complexity theory for dynamic problems in the bit-probe/cell-probe model of computation. We now mention a couple of concrete implications that follow from this study.






Consider  the {\em dynamic Orthogonal Vector} (OV) problem (see \Cref{main:def:OV}). Lower bounds conditional on SETH for many natural problems (e.g.  Subgraph connectivity, ST-reachability, Chan's subset union,  3-vs-4 Diameter) are based on reductions from dynamic OV~\cite{AbboudW14}.
This suggests two research directions: (I) Prove strong {\em unconditional} lower bounds for many natural problems in one shot by proving a polynomial cell-probe lower bound for dynamic OV. (II) Prove lower bounds conditional on SETH for the family of connectivity problems mentioned in the previous page via reductions (in the word RAM model) from dynamic OV. 
Below are some questions about the feasibility of these research directions that our theory can answer. We are not aware of any other technique in the existing literature that can provide similar conclusions.




\smallskip
\noindent {\bf (I) What if dynamic OV is easy in the cell-probe model?}
For the first direction, there is a risk that dynamic OV might turn out to admit a polylogarithmic update time algorithm in the cell-probe model. This is because  lower bounds  in the word RAM model do not necessarily extend to the cell-probe model. For example, it was shown by Larsen and Williams~\cite{LarsenW17} that the OMv conjecture \cite{OMV} is false in the cell-probe model. 

Will all the efforts be wasted if dynamic OV turns out to admit polylogarithmic update time in the cell-probe model? Our theory implies that this will also lead to a very interesting algorithmic consequence: If dynamic OV admits polylogarithmic update time in the cell-probe model, so do several important dynamic problems such as $k$-edge connectivity,  $(1+\epsilon)$-approximate mincut, $(1+\epsilon)$-approximate matching, planar nearest neighbors, Chan's subset union and 3-vs-4 diameter.
The same conclusion can be made when we replace dynamic OV by, e.g., subgraph connectivity, single source reachability, Chan's subset union, and 3-vs-4 diameter (see \Cref{thm:intro:results_summary}). 
Thus, there will be interesting consequences regardless of the outcome of this line of research.

Roughly, the conclusion above can be made by proving in the dynamic setting an analogue of the fact (in the static setting) that if P=NP, then the polynomial hierarchy (PH) collapses. This is done by carefully defining the classes $\dP$, $\dNP$ and $\dPH$ as dynamic analogues of P, NP, and PH, so that we can prove such collapse and prove $\dNP$-completeness and $\dNP$-hardness results for natural dynamic problems, including dynamic OV. We sketch how to do this in \Cref{sec:intro:contribution,sec:overview}. 




\smallskip
\noindent {\bf (II) Lower bounds for $k$-edge connectivity via dynamic OV?} As discussed above, whether dynamics $k$-edge connectivity admits  polylogarithmic update time for  $k\in [3, O(\log n)]$  is a very important open question. There is  a hope to answer this question negatively via reductions (in the word RAM model) from dynamic OV. 

Our theory provides a method to refute such a possibility (the so-called {\em non-reducibility}). First, note that any reduction from dynamic OV in the word RAM model will also hold in the (stronger) cell-probe model. Armed with this simple observation, we show that there are no ``efficient'' reductions from dynamic OV to $k$-edge connectivity under an assumption about the complexity classes for dynamic problems in the cell-probe model, namely $\dPH \not\subseteq \dMA \cap \dcoMA$ (see \Cref{thm:intro:ruleout_reductions}). We defer defining the classes $\dMA$ and $\dcoMA$, but note two things. (i) Just as the classes MA and  coMA (where MA stands for {\em Merlin-Arthur}) extend NP in the static setting, the classes $\dMA$ and $\dcoMA$ extend the class $\dNP$ in a similar manner. (ii) In the static setting it is widely believed that PH $\not\subseteq$ MA $\cap$ coMA because otherwise the PH collapses.
Here, {\em efficient reduction} from problems $X$ to $Y$ roughly refers to a way to process each update for problem $X$ by quickly making polylogarithmic number of updates to an algorithm for $Y$. (See \Cref{sec:reduction} for details.)
All reductions from dynamic OV in the literature that we are aware of are efficient reductions.\footnote{Note that we define our complexity classes in the cell-probe model, whereas the reductions from dynamic OV are in the word RAM model. This does not make any difference, however, since any reduction in the  word RAM reduction continues to have the same  guarantees in the (stronger) cell-probe model.}


To show a similar result for any problem $X$, one needs to prove that $X\in \dMA \cap \dcoMA$, which boils down to developing efficient randomized {\em verification protocols} for such problems. We explain this in more details in \Cref{sec:intro:contribution} and  \Cref{sec:rand_classes}.


We are not aware of any existing assumptions that can lead the same conclusion as above. 
To our knowledge, the only conjecture that can imply results of this nature is the  Nondeterministic Strong Exponential Time Hypothesis (NSETH) of~\cite{CarmosinoGIMPS16}. However, it needs a stronger property of $k$-edge connectivity that is not yet known to be true,\footnote{In particular, \Cref{thm:intro:ruleout_reductions} follows from the fact that $k$-edge connectivity is in  $\dMA \cap \dcoMA$. To use NSETH, we need to show that it is in $\dNP\cap \dcoNP$.} and even with such a property it would only rule out deterministic reductions since NSETH only holds for deterministic algorithms.


\smallskip
\noindent {\bf Paper Organization.} In \Cref{sec:intro:contribution}, we explain our contributions in details, including the conclusions above and beyond. We discuss related works and future directions in \Cref{sec:related:work,sec:open}. An overview of our main technical proof, the $\dNP$-completeness, is in \Cref{sec:overview}. In \Cref{part:formalization} we formalize required notions. Although some of them are tedious, they are crucial to get things right. \Cref{part:completeness} provides detailed proofs of our $\dNP$-completeness results. \Cref{part:further_classes} extends our study to other classes, including those with randomization. This is needed for the non-reducibility result mentioned above, discussed in details in \Cref{part:connectivity}. 




\endinput

============================
============================
============================

{\color{red}
xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
}




For example, one reason that makes the $P\neq NP$ assumption so central in the static setting is that proving and disproving it will both lead to stunning consequences: 
If the assumption is false then hundreds of problems in NP and bigger complexity classes like the polynomial hierarchy (PH) admit efficient algorithms; otherwise the situation will be the opposite.\footnote{For further consequences see, e.g., \cite{Aaronson17,Cook2006p,Cook03} and references therein.}
 
In contrast, we do not see any immediate consequence to dynamic algorithms if someone falsified SETH, OMv, or any other assumptions.\footnote{An indirect consequence would be that some barriers were broken and we might hope to get better upper bounds. This is however different from when P=NP where many hard problems would immediately admit efficient algorithms. Note that some consequences of falsifying SETH have been shown recently (e.g. \cite{AbboudBDN18,Williams13,GaoIKW17,CyganDLMNOPSW16,SanthanamS12,JahanjouMV15,DantsinW13}); however, we are not aware of any consequence to dynamic algorithms. It might also be interesting to note that Williams~\cite{Williams18-likelihood} estimates the likelihood of SETH to be only 25\%.}
As another example, comparing complexity classes allows us to speculate on various situations such as non-reducibility (e.g. \cite{AharonovR05,KlivansM02,Condon92}), the existence of NP-intermediate problems \cite{Ladner75} and the derandomization possibilities (e.g. \cite{ImpagliazzoW97}). (See more in \Cref{sec:open}.)
We cannot anticipate results like these in the dynamic setting without the coarse-grained approach, i.e. by considering analogues of P, NP, BPP and other complexity classes that are defined based on computational resources. 




Since dynamic algorithms and (coarse-grained) computational complexity have coexisted with each other for several decades, it is only natural that some attempts were made in the past towards building a complexity theory for dynamic problems (see~\ref{sec:related:work} for  more details). Nevertheless, we are not aware of any existing result that implies  (super-polylogarithmic) hardness of  well-known dynamic problems via a  coarse-grained approach. 










==> open.tex <==
\section{Future Directions}\label{sec:open}


One byproduct of our paper is a way to prove non-reducibility.
It is interesting to use this method to shed more light on the hardness of other dynamic problems. To do so, it suffices to show that such problem is in  $\dMA \cap \dcoMA$ (or, even better, in $\dNP\cap \dcoNP$). One particular problem is whether connectivity is in $\dNP\cap \dcoNP$. It is known to be in $\dMA \cap \dcoMA$ due to the randomized algorithm of Kapron~et~al \cite{KapronKM13}. It is also in $\dNP$ (see \Cref{ex:intro:connectivity in NP}). The main question is whether it is in  $\dcoNP$. (Techniques from \cite{NanongkaiSW17,Wulff-Nilsen17,NanongkaiS17} almost give this, with verification time $n^{o(1)}$  instead of polylogarithmic.) Having connectivity in  $\dNP\cap \dcoNP$ would be a strong evidence that it is in $\dP$, meaning that it admits a deterministic algorithm with polylogarithmic update time. Achieving such algorithm will be a major breakthrough. Another specific question is whether the promised version of the $(2-\epsilon)$ approximate matching problem is in $\dMA\cap \dcoMA$. This would rule out efficient reductions from dynamic OV to this problem. Whether this problem admits a randomized algorithm with polylogarithmic update time is a major open problem. 
Other problems that can be  studied in this direction include approximate minimum spanning forest (MSF), $d$-weight MSF, bipartiteness, 
dynamic set cover, dominating set, and $st$-cut.

It is also very interesting to rule out efficient reductions from the following variant of the OuMv conjecture: At the preprocessing, we are given a boolean $n\times n$ matrix $M$ and boolean $n$-dimensional row and column vectors $u$ and $v$. Each update changes one entry in either $u$ or $v$. We then have to output the value of $uMv$. Most lower bounds that are hard under the OMv conjecture \cite{OMV} are via efficient reductions from this problem. It is interesting to rule out such efficient reductions since SETH and OMv are two conjectures that imply most lower bounds for dynamic problems.





Now that we can prove completeness and relate some basic complexity classes of dynamic problems, one big direction to explore is whether more results from coarse-grained complexity for static problems can be reconstructed for dynamic problems. Below are a few samples. 



\begin{enumerate}[noitemsep]
\item {\em Derandomization:} Making dynamic algorithms deterministic is an important issue. Derandomization efforts have so far focused on specific problems (e.g. \cite{NanongkaiS17,NanongkaiSW17,BernsteinC16,BernsteinC17,Bernstein17,BhattacharyaHI18,BhattacharyaCHN18-coloring,BhattacharyaHN16}). Studying this issue via the class $\dBPP$ might lead us to the more general understanding. 
For example, the {\em Sipser-Lautermann theorem} \cite{Sipser83a,Lautemann83} states that $BPP\subseteq \Sigma _{2}\cap \Pi _{2}$, Yao \cite{Yao82a} showed that the existence of some pseudorandom generators would imply that $P = BPP$, and Impagliazzo and Wigderson \cite{ImpagliazzoW97} suggested that $BPP=P$ (assuming that any problem in $E =DTIME(2^{O(n)})$ has circuit complexity $2^{\Omega(n)}$).  We do not know anything similar to these for dynamic problems.  

	


\item {\em NP-Intermediate:} Many static problems (e.g. graph isomorphism and factoring) are considered good candidates for being NP-intermediate, i.e. being neither in P nor NP-complete. This paper leaves many natural problems in $\dNP$ unproven to be $\dNP$-complete. Are these problems in fact $\dNP$-intermediate? The first step towards this question might be proving an analogues of {\em Ladner's theorem} \cite{Ladner75}, i.e. that an $\dNP$-intermediate dynamic problem exists, assuming $\dP\neq \dNP$. 
It is also interesting to prove the analogue of the {\em time-hierarchy theorems}, i.e. that with more time, more dynamic problems can be solved. (Both theorems are proved by diagonalization in the static setting.)




\item This work and lower bounds from fine-grained complexity has focused mostly on {\em decision}  problems. There are also {\em search dynamic problems}, which always have valid solutions, and the challenge is how to maintain them. These problems include maximal matching, maximal independent set, minimal dominating set, coloring vertices with  $(\Delta+1)$ or more colors, and coloring edges with $(1+\epsilon)\Delta$ or more colors, where $\Delta$ is the maximum degree (e.g. \cite{BaswanaGS15,BhattacharyaCHN18-coloring,AssadiOSS18-MIS,SolomonW18-coloring,DuZ18,GuptaK18,OnakSSW18}).  These problems  do not seem to correspond to any decision problems. Can we define complexity classes for these problems and argue that some of them might not admit polylogarithmic update time? Analogues of TFNP and its subclasses (e.g. PPAD) might be helpful here.
\end{enumerate}

\noindent There are also other concepts that have not been discussed in this paper at all, such as interactive proofs, probabilistically checkable proofs (PCP), counting problems (e.g. Toda's theorem), relativization and other barriers. Finally, in this paper we did not discuss amortized update time. It is a major open problem whether similar results, especially an analogue of NP-hardness, can be proved for algorithms with amortized update time.






\endinput

\section{OLD Open Problems}
\begin{itemize}
\item Is dynamic connectivity in $\dP$? 

\begin{itemize}
\item Best known: KKM, NWS, Holm et al
\item Will imply that dynamic $k$-edge connectivity is in $\dcoNP$.
\item Prerequisite: show that dynamic cycle detection is in $\dP$.
\end{itemize}
\item Is dynamic $2$-approximate maximum matching in $\dP$ or $\dBPP$
?
\item Is dynamic planar nearest neighbor in $\dP$ or $\dBPP$?

\begin{itemize}
\item Best known: \cite{Chan10,ChanT16} $polylog(n)$ deterministic amortized
\end{itemize}
\item Possible to show a completeness for $\dNP$?

\begin{itemize}
\item how about in RAM? can we remove the relaxation about quasi-polynomial
time?
\end{itemize}
\item Can we show a complete problem of $\dNP$ in the RAM model without
relaxation on the preprocessing time?\end{itemize}



==> overview.tex <==
\section{An Overview of the $\dNP$-Completeness Proof}
\label{sec:overview}


In this section, we present an overview of one of our main technical contributions (the proof of~\ref{thm:intro:DNF}) at a finer level of granularity.   In order to explain the main technical insights we focus on a nonuniform model of computation called the \emph{bit-probe} model, which has been studied
since the 1970's~\cite{Fredman78, Miltersen99cellprobe}.  













\subsection{Dynamic Complexity Classes $\dP$ and $\dNP$}
\label{main:sec:class}







We begin by reviewing (informally) the concepts of a dynamic problem and an algorithm in the bit-probe model. See~\ref{sec:model} for a formal description.
Consider any dynamic problem $\D_n$. Here, the subscript $n$ serves as a reminder that the bit-probe model is nonuniform and it also indicates that each  instance $I$ of this problem can be specified using $n$ bits. We will will mostly be concerned with dynamic {\em decision} problems, where the {\em answer} $\D_n(I) \in \{0,1\}$ to every instance $I$ can be specified using a single bit. We say that $I$ is an YES instance if $\D_n(I) = 1$, and a NO instance if $\D_n(I) = 0$. An algorithm $\A_n$ for this dynamic problem $\D_n$ has access to a memory $\mem_n$, and the total number of bits available in this memory is called the {\em space complexity} of $\A_n$.  The algorithm $\A_n$ works in steps $t = 0, 1, \ldots,$ in the following manner.



\medskip
\noindent {\em Preprocessing:} At step $t = 0$ (also called the preprocessing step), the algorithm gets a {\em starting instance} $I_0 \in \D_n$ as input. Upon receiving this input, it initializes the bits in its memory $\mem_n$ and then it {\em outputs} the {\em answer} $\D_n(I_0)$ to the {\em current instance} $I_0$.

\medskip
\noindent {\em Updates:} Subsequently, at each step $t \geq 1$, the algorithm gets an {\em instance-update} $(I_{t-1}, I_t)$ as input. The sole purpose of this instance-update is to change the current instance  from $I_{t-1}$ to $I_t$. Upon receiving this input, the algorithm probes (reads/writes) some bits in the memory $\mem_n$, and then outputs the answer $\D_n(I_t)$ to the  current instance $I_t \in \D_n$. The {\em update time} of  $\A_n$ is the maximum number of bit-probes it needs to make in $\mem_n$ while handling an instance-update.

\medskip
One way  to visualize the above description as follows. An adversary keeps constructing an {\em instance-sequence} $(I_0, I_1, \ldots, I_k, \ldots)$  one step at a time. At each step $t$, the algorithm $\A_n$ gets the corresponding instance-update $(I_{t-1}, I_t)$, and at this point it is only aware of the prefix $(I_0, \ldots, I_t)$. Specifically, the algorithm does not know the future instance-updates. After receiving the instance-update at each step $t$, the algorithm has to output the answer to the current instance $\D_n(I_t)$. 




The above framework is flexible enough to capture dynamic problems that allow for both {\em update} and {\em query} operations, because we can easily model a query operation as an instance-update. This fact is illustrated in more details in~\ref{exa:query}. Furthermore, throughout this paper w.l.o.g. we assume that an instance-update in a dynamic problem $\D_n$ can be specified using $O(\log n)$ bits. See the discussion preceding~\ref{assume:logn update size} for a more detailed explanation of this phenomenon. 



For technical reasons, we will work under the following assumption. This assumption will be implicitly present in the definitions of the complexity classes $\dP$ and $\dNP$ below.

\begin{assumption}
 \label{assume:poly:main}
A dynamic algorithm $\A_n$ for a dynamic problem $\D_n$ has to handle at most $\poly(n)$ many instance-updates.
 \end{assumption}

We are now ready to define  the complexity class $\dP$. 




\begin{defn}
[Class $\dP$]\label{main:def:P} A dynamic decision problem $\D_n$ is in $\dP$ iff there is an algorithm $\A_n$
solving $\D_n$ which has update time $O(\polylog (n))$ and space-complexity $O(\poly (n))$.
\end{defn}





In order to define the  class $\dNP$, we first introduce the notion of a {\em verifier} in~\ref{main:def:verifier}. Subsequently, we introduce the class $\dNP$ in~\ref{main:def:NP}. We have already discussed the intuitions behind these concepts in~\ref{sec:intro} after the statement of~\ref{def:intro:dNP}.


\begin{defn}[Dynamic verifier]
\label{main:def:verifier}
We say that a dynamic algorithm $\V_n$ with space-complexity $O(\poly (n))$ is a {\em verifier} for a dynamic decision problem $\D_n$ iff it works as follows.

\smallskip
\noindent {\em Preprocessing:} At step $t = 0$, the algorithm $\V_n$ gets a {\em starting instance} $I_0 \in \D_n$ as input, and it outputs an ordered pair $(x_0, y_0)$ where $x_0 \in \{0,1\}$ and $y_0 \in \{0,1\}^{\polylog(n)}$.

\smallskip
\noindent {\em Updates:} Subsequently, at each step $t \geq 1$, the algorithm $\V_n$ gets an {\em instance-update} $(I_t, I_{t-1})$ and a {\em proof} $\pi_t \in \{0,1\}^{\polylog (n)}$ as input, and it outputs an ordered pair $(x_t, y_t)$ where $x_t \in \{0,1\}$ and $y_t \in \{0,1\}^{\polylog (n)}$. The algorithm $\V_n$ has $O(\polylog (n))$ update time, i.e., it makes at most $O(\polylog (n))$ bit-probes in the memory during each step $t$. Note that the output $(x_t, y_t)$ depends on  the instance-sequence $(I_0, \ldots, I_t)$  and the {\em proof-sequence} $(\pi_1, \ldots, \pi_t)$ seen so far. 
\end{defn}




\begin{defn}
[Class $\dNP$]\label{main:def:NP} A decision problem $\D_n$ is in $\dNP$ iff it admits a verifier $\V_n$ which satisfy the following properties.  Fix any instance-sequence $(I_0, \ldots, I_k)$. Suppose that the verifier  $\V_n$ gets $I_0$ as input at step $t = 0$ and the ordered pair $((I_{t-1},I_t), \pi_t)$ as input at every step $t \geq 1$. Then:
\begin{enumerate}
\item  For every proof-sequence $(\pi_1, \ldots, \pi_k)$,  we have  $x_t = 0$ for each $t \in \{0, \ldots, k\}$ where $\D_n(I_t) = 0$.
\item If the proof-sequence $(\pi_1, \ldots, \pi_k)$ is {\em reward-maximizing} (defined below), then we have $x_t = 1$ for each $t \in \{0, \ldots, k\}$ with $\D_n(I_t) = 1$, 
\end{enumerate}
The proof-sequence $(\pi_1, \ldots, \pi_k)$ is {\em reward-maximizing} iff the following holds.  At each step $t \geq 1$, given the past history $(I_0, \ldots, I_t)$ and $(\pi_1, \ldots, \pi_{t-1})$, the proof $\pi_t$ is chosen in such a way that maximizes the value of $y_t$. We say that such a proof $\pi_t$ is {\em reward-maximizing}.
\end{defn}


Just as in the static setting, we can easily prove that $\dP \subseteq \dNP$ and we conjecture that $\dP \neq \dNP$. The big question left open in this paper is to resolve this conjecture.

\begin{cor}
\label{main:cor:pnp}
We have $\dP \subseteq \dNP$.
\end{cor}









\subsection{A complete problem in $\dNP$}
\label{main:sec:complete}

One of the main results in this paper shows that a natural  problem called {\em dynamic narrow DNF evaluation} (denoted by $\dDNF$) is $\dNP$-complete. Intuitively, this means that (a) $\dDNF \in \dNP$, and (b) if $\dDNF \in \dP$ then $\dP = \dNP$.\footnote{To be more precise, condition (b) means that  every problem in $\dP$ is $\dP$-reducible to $\dDNF$. See~\ref{sec:reduction} for a formal definition.} We now give an informal description of this problem.  

\medskip
\noindent {\bf Dynamic narrow DNF evaluation ($\dDNF$):} An instance $I$ of this problem consists of a triple $(\Z, \C, \phi)$, where $\Z = \{z_1, \ldots, z_N\}$ is a set of $N$ variables,  $\C = \{ C_1, \ldots, C_M\}$ is a set of $M$ DNF clauses, and  $\phi : \Z \rightarrow \{0,1\}$ is an assignment of values to the variables. Each clause $C_j$ is a conjunction (AND) of at most $\polylog (N)$ literals, where each literal is of the form $z_i$ or $\neg z_i$ for some variable  $z_i \in \Z$. This is an YES instance if   at least one clause $C \in \C$  is true under the assignment $\phi$, and this is a NO instance if every clause in $\C$ is false under the assignment $\phi$. Finally, an {\em instance-update}  changes the assignment $\phi$ by flipping the value of exactly one variable in $\Z$. 


It is easy to see that the above problem is in $\dNP$. Specifically, if the current instance is an YES instance, then a proof $\pi_t$ simply points to a specific clause $C_j \in \C$ that is true under the current assignment $\phi$. The proof $\pi_t$ can be encoded using $O(\log M)$ bits. Furthermore, since each clause contains at most $\polylog (N)$ literals, the verifier can check that the clause $C_j$ specified by the proof $\pi_t$ is true under the assignment $\phi$ in $O(\polylog (N))$ time. On the other hand, no proof can fool the verifier if the current instance is a NO instance (where every clause is false). All these observations can be formalized in a manner consistent with~\ref{main:def:NP}. We will prove the following theorem.

\begin{thm}
\label{main:thm:NP:complete}
The $\dDNF$ problem described above is $\dNP$-complete.
\end{thm}

In order to prove~\ref{main:thm:NP:complete}, we consider an intermediate dynamic problem called $\fDNF$. 


\medskip
\noindent {\bf $\fDNF$:} An instance $I$ of $\fDNF$ consists of a tuple $(\Z, \C, \phi, \prec)$. Here, the symbols $\Z, \C$ and $\phi$ denote exactly the same objects as in the $\dDNF$ problem described above. In addition, the symbol $\prec$ denotes a total order on the set of clauses $\C$. The answer to this instance $I$ is defined as follows. If every clause in $\C$ is false under the current assignment $\phi$, then the answer to $I$ is $0$. Otherwise, the answer to $I$ is the {\em first clause}  $C_j \in \C$ according to the total order $\prec$ that is true under $\phi$. It follows that $\fDNF$ is {\em not} a decision problem.  Finally, as before, an instance-update for the $\fDNF$  changes the assignment $\phi$ by flipping the value of exactly one variable in $\Z$.



\medskip
 We prove~\ref{main:thm:NP:complete} as follows. (1) We first show that  $\fDNF$ is $\dNP$-hard. Specifically, if there is an algorithm for $\fDNF$ with polylog update time and polynomial space complexity, then $\dP = \dNP$. We explain this in more details in~\ref{main:sec:NP:hard}. (2) Using a standard binary-search trick, we show that there exists an $O(\polylog (n))$ time {\em reduction} from $\fDNF$ to $\dDNF$. Specifically, this means that if $\dDNF \in \dP$, then we can use an algorithm for $\dDNF$ as a subroutine to design an algorithm for $\fDNF$ with polylog update time and polynomial space complexity.~\ref{main:thm:NP:complete} follows from (1) and (2), and the observation that $\dDNF \in \dNP$.

\subsubsection{$\dNP$-hardness of $\fDNF$}
\label{main:sec:NP:hard}

Consider any dynamic decision problem $\D_n \in \dNP$. Thus, there exists a verifier $\V_n$ for $\D_n$ with the properties mentioned in~\ref{main:def:NP}. Throughout~\ref{main:sec:NP:hard}, we assume that  there is an algorithm for $\fDNF$ with polynomial space complexity and polylog update time. Under this assumption, we will show that there exists an algorithm $\A_n$ for $\D_n$ that also has $O(\poly (n))$ space complexity and $O(\polylog (n))$ update time. This will imply the $\dNP$-hardness of $\fDNF$.

\medskip
\noindent {\bf The high-level strategy:} The algorithm $\A_n$ will use the following two {\em subroutines}: (1) The verifier $\V_n$ for $\D_n$ as specified in~\ref{main:def:verifier} and~\ref{main:def:NP}, and (2) A dynamic algorithm $\A^*$ that solves the $\fDNF$ problem with polylog update time and polynomial space complexity.   

To be more specific, consider any instance-sequence $(I_0, \ldots, I_k)$ for the problem $\D_n$. At step $t = 0$, after receiving the starting instance $I_0$, the algorithm $\A_n$ calls the subroutine $\V_n$ with the same input $I_0$. The subroutine $\V_n$ returns an ordered pair $(x_0, y_0)$. At this point, the algorithm $\A_n$ outputs the bit $x_0$. Subsequently, at each step $t \geq 1$, the algorithm $\A_n$ receives the instance-update $(I_{t-1}, I_t)$ as input. It then calls the subroutine $\A^*$ in such a manner which ensures that $\A^*$ returns a reward-maximizing proof $\pi_t$ for the verifier $\V_n$ (see~\ref{main:def:NP}). This is explained in more details below. The algorithm $\A_n$ then calls the verifier $\V_n$ with the input $((I_{t-1}, I_t), \pi_t)$, and the verifier returns an ordered pair $(x_t, y_t)$. At this point, the algorithm $\A_n$ outputs the bit $x_t$.

To summarize, the algorithm $\A_n$ uses $\A^*$ as a dynamic subroutine to construct a reward-maximizing proof-sequence $(\pi_1, \ldots, \pi_k)$ -- one step at a time. Furthermore, after each step $t \geq 1$, the algorithm $\A_n$ calls the verifier $\V_n$ with the input $((I_{t-1}, I_t), \pi_t)$. The verifier $\V_n$ returns $(x_t, y_t)$, and the algorithm $\A_n$ outputs $x_t$. Item (1) in~\ref{main:def:NP} implies that the algorithm $\A_n$ outputs $0$ on all the NO instances (where $\D_n(I_t) = 0$). Since the proof-sequence $(\pi_1, \ldots, \pi_k)$ is reward-maximizing, item (2) in~\ref{main:def:NP} implies that the algorithm $\A_n$ outputs $1$ on all the YES instances (where $\D_n(I_t) = 1$). So the algorithm $\A_n$ always outputs the correct answer and solves the problem $\D_n$. We now explain how the algorithm $\A_n$ calls the subroutine $\A^*$, and then analyze the space complexity and update time of $\A_n$. The key observation is that we can represent  the verifier $\V_n$ as a collection of decision trees, and each root-to-leaf path in each of these  trees can be modeled as a DNF clause.\footnote{Give citations.}


\medskip
\noindent {\bf The decision trees that define the verifier $\V_n$:}
Let $\mem_{\V_n}$ denote the memory of the verifier $\V_n$. We assume that during each step $t \geq 1$, the instance-update $(I_{t-1}, I_t)$ is written in a designated region $\mem_{\V_n}^{(0)} \subseteq \mem_{\V_n}$ of the memory, and the proof $\pi_t$ is written in another designated region $\mem_{\V_n}^{(1)} \subseteq \mem_{\V_n}$ of the memory. Each bit in $\mem_{\V_n}$ can be thought of as a boolean variable $z \in \{0,1\}$. We view the region $\mem_{\V_n} \setminus \mem_{\V_n}^{(1)}$ as a collection of boolean variables $\Z = \{ z_1, \ldots, z_N \}$ and the contents of $\mem_{\V_n} \setminus \mem_{\V_n}^{(1)}$ as an assignment $\phi : \Z \rightarrow \{0,1\}$. For example, if $\phi(z_j) = 1$ for some $z_j \in \Z$, then it means that the bit $z_j$ in $\mem_{\V_n} \setminus \mem_{\V_n}^{(1)}$ is currently set to $1$. Upon receiving an input $((I_{t-1}, I_t), \pi_t)$, the verifier $\V_n$ makes some probes in $\mem_{\V_n} \setminus \mem_{\V_n}^{(1)}$ according to some pre-defined procedure, and then outputs an answer $(x_t, y_t)$. This procedure can be modeled as a decision tree $T_{\pi_t}$. Each internal node (including the root) in this decision tree is either a "read" node  or a "write" node. Each read-node has two children and is labelled with a variable $z \in \Z$. Each write-node has one child and is labelled with an ordered pair $(z, \lambda)$, where $z \in \Z$ and $\lambda \in \{0,1\}$. Finally, each leaf-node of $T_{\pi_t}$ is labelled with an ordered pair $(x, y)$, where $x \in \{0,1\}$ and $y \in \{0,1\}^{\polylog (n)}$.  Upon receiving the input $((I_{t-1}, I_t), \pi_t)$, the verifier $\V_n$ {\em traverses} this decision tree $T_{\pi_t}$. Specifically, it starts at the root of $T_{\pi_t}$, and then inductively applies the following steps until it reaches a leaf-node. 
\begin{itemize}
\item Suppose that it is currently at a read-node of $T_{\pi_t}$  labelled with $z \in \Z$. If $\phi(z) = 0$ (resp. $\phi(z) = 1$), then it goes to the left (resp. right) child of the node. On the other hand, suppose that it is currently at a write-node of $T_{\pi_t}$ which is labelled with $(z, \lambda)$. Then it writes $\lambda$ in the memory-bit $z$ (by setting $\phi(z) = \lambda$) and then moves on to the only child of this node. 
\end{itemize}
Finally, when it reaches a leaf-node, the verifier $\V_n$ outputs the corresponding label $(x, y)$. This is the way the verifier operates when it is called with an input $((I_{t-1}, I_t), \pi_t)$. The depth of the decision tree (the maximum length of any root-to-leaf path) is at most $\polylog (n)$, since as per~\ref{main:def:verifier} the verifier makes at most $\polylog (n)$ many bit-probes in the memory while handling any input.  

Each possible proof $\pi$ for the verifier can be specified using $\polylog (n)$ bits. Hence, we get a collection of $O(2^{\polylog (n)})$ many decision trees $\T = \{ T_{\pi} \}$ -- one tree $T_{\pi}$ for each possible input $\pi$. This collection of decision trees $\T$ completely characterizes the verifier $\V_n$.

\medskip
\noindent {\bf DNF clauses corresponding to a decision tree $T_{\pi_t}$:} Suppose that the proof $\pi$ is given as part of the input to the verifier during some update step. Consider any root-to-leaf path $P$ in a decision tree $T_{\pi}$. We can naturally associate a DNF clause $C_P$  corresponding to this path $P$. To be more specific, suppose that the path $P$ traverses a read-node labelled with $z \in \Z$ and then goes to its left (resp. right) child. Then we have a literal $\neg z$ (resp. $z$) in the clause $C_P$ that corresponds to this read-node.\footnote{W.l.o.g. we can assume that no two read nodes on the same path are labelled with the same variable.} The clause $C_P$ is the conjunction (AND) of these literals, and $C_P$ is true iff the verifier $\V_n$ traverses the path $P$ when $\pi$ is the proof given to it as part of the input. Let $\C = \{ C_P : P \text{ is a root-to-leaf path in some tree } T_{\pi} \in \T \}$ be the collection of all these DNF clauses. 

\medskip
\noindent {\bf Defining a total order $\prec$ over $\C$:} We now define a total order $\prec$ over $\C$ which satisfies the following property: Consider any two root-to-leaf paths $P$ and $P'$ in the collection of decision trees $\T$. Let $(x, y)$ and $(x', y')$ respectively denote the labels associated with the leaf nodes of the paths $P$ and $P'$. If $C_{P} \prec C_{P'}$, then $y \geq y'$.  Thus, the paths with higher $y$ values appear earlier in $\prec$. 

\medskip
\noindent {\bf Finding a reward-maximizing proof:} Suppose that $(I_0, \ldots, I_{t-1})$ is the instance-sequence of $\D_n$ received by $\A_n$ till now. By induction, suppose that  $\A_n$ has managed to construct a reward-maximizing proof-sequence $(\pi_1, \ldots, \pi_{t-1})$ till this point, and has fed this as input to the verifier $\V_n$ (which is used as a subroutine). At the present moment, suppose that $\A_n$ receives an instance-update $(I_{t-1}, I_t)$ as input. Our goal now is  to find a reward-maximizing proof $\pi_t$ at the current step $t$.


Consider the tuple $(\Z, \C, \phi, \prec)$ where $\Z = \mem_{\V_n} \setminus \mem_{\V_n}^{(1)}$ is the set of variables, $\C = \{ C_P : P \text{ is a root-to-leaf path in some decision tree } T_{\pi}\}$ is the set of DNF clauses,  the assignment $\phi : \Z \rightarrow \{0,1\}$ reflects the current contents of the memory-bits in $\mem_{\V_n} \setminus \mem_{\V_n}^{(1)}$, and $\prec$ is the total ordering over $\C$ described above.  Let $C_{P'} \in \C$ be the answer to this $\fDNF$ instance $(\Z, \C, \phi, \prec)$, and suppose that the path $P'$ belongs to the decision tree $T_{\pi'}$ corresponding to the proof $\pi'$. A moment's thought will reveal that $\pi_t = \pi'$ is the desired reward-maximizing proof at step $t$ we were looking for, because of the following reason. Let $(x', y')$ be the label associated with the leaf-node in $P'$. By definition, if the verifier gets the ordered pair $((I_{t-1}, I_t), \pi')$ as input at this point, then  it will traverse the path $P'$ in the decision tree $T_{\pi'}$ and return the ordered pair $(x', y')$. Furthermore, the path $P'$ comes first according to the total ordering $\prec$, among all the paths that can be traversed by the verifier at this point. Hence, the path $P'$ is chosen in such a way that maximizes $y'$, and accordingly, we conclude that $y_t = y'$ is a reward-maximizing proof at step $t$. 

\medskip
\noindent {\bf Wrapping up: Handling an instance-update $(I_{t-1}, I_t)$.} To summarize, when the algorithm $\A_n$ receives an instance-update $(I_{t-1}, I_t)$, it works as follows. It first writes down in the instance-update $(I_{t-1}, I_t)$ in $\mem_{\V_n}^{(0)}$ and accordingly updates the assignment $\phi : \Z \rightarrow \{0,1\}$. It then calls the subroutine $\A^*$ on the $\fDNF$ instance $(\Z, \C, \phi, \prec)$. The subroutine $\A^*$ returns a reward-maximizing proof $\pi_t$. The algorithm $\A_n$ then calls the verifier $\V_n$ as a subroutine with the ordered pair $((I_{t-1}, I_t), \pi_t)$ as input. The verifier updates at most $\polylog (n)$ many bits in $\mem_{\V_n}$  and returns an ordered pair $(x_t, y_t)$. The algorithm $\A_n$ now  updates the assignment $\phi : \Z \rightarrow \{0,1\}$ to ensure that it is synchronized with the current contents of  $\mem_{\V_n}$. This requires $O(\polylog (n))$ many calls to the subroutine $\A^*$ for the $\fDNF$ instance. Finally,  $\A_n$ outputs the bit $x_t \in \{0,1\}$.

\medskip
\noindent {\bf Bounding the update time of $\A_n$:} 
Notice that after each instance-update $(I_{t-1}, I_t)$, the algorithm $\A_n$ makes one call to the verifier $\V_n$ and at most $\polylog (n)$ many calls to $\A^*$. By~\ref{main:def:verifier}, the call to  $\V_n$ requires $O(\polylog (n))$ time. Furthermore, we have assumed that  $\A^*$ has polylog update time. Hence, each call to $\A^*$ takes $O(\polylog (N, M)) = O(\polylog (2^{\polylog (n)})) = O(\polylog (n))$ time. Since the algorithm $\A_n$ makes at most $\polylog (n)$ many calls to $\A^*$, the total time spent in these calls is still $O(\polylog (n))$. Thus, we conclude that  $\A_n$ has $O(\polylog (n))$ update time. 



\renewcommand{\S}{\mathcal{S}}

\medskip
\noindent {\bf Bounding the space complexity of $\A_n$:} The space complexity of $\A_n$ is dominated by the space complexities of the subroutines $\V_n$ and $\A^*$. As per~\ref{main:def:verifier},   the verifier $\V_n$ has space complexity $O(\poly (n))$.


We next bound the memory space used by the subroutine $\A^*$. Note that in the $\fDNF$ instance, we have a DNF clause $C_P \in \C$ for every root-to-leaf path $P$ of every decision tree $T_{\pi}$. Since a proof $\pi$ consists of $\polylog (n)$ bits, there are at most $O(2^{\polylog (n)})$ many decision trees of the form $T_{\pi}$. Furthermore,  since every root-to-leaf path is of length at most $\polylog (n)$, each decision tree $T_{\pi}$ has at most $O(2^{\polylog (n)})$ many root-to-leaf paths. These two observations together imply that the set of clauses $\C$ is of size at most $O\left(2^{\polylog (n)} \cdot 2^{\polylog (n)}\right) = O(2^{\polylog (n)})$. Furthermore, as per~\ref{main:def:verifier} there are at most $O(\poly (n))$ many bits in the memory $\mem_{\V_n}$, which means that there are at most $O(\poly (n))$ many variables in $\Z$. Thus, the $\fDNF$ instance $(\Z, \C, \phi, \prec)$ is defined over a set of $N = \poly (n)$ variables and a set of $M = 2^{\polylog (n)}$ clauses (where each clause consists of at most $\polylog (n)$ many literals).  We have assumed that $\A^*$ has quasipolynomial space complexity. Thus, the total space needed by the subroutine $\A^*$ is $O(2^{\polylog (N, M)}) = O(2^{\polylog (n)})$. 

Unfortunately, the bound of $2^{\polylog (n)}$ is too large for us. Instead, we will like to have a space complexity of $O(\poly (n))$. Towards this end, we introduce a new subroutine $\S^*_n$ that acts as an {\em interface} between the subroutine $\A^*$ and the memory $\mem_{\A^*}$ used by $\A^*$ (see~\ref{sec:cor:np-hardness} for details). Specifically, as we observed in the preceding paragraph, the memory $\mem_{\A^*}$ consists of $2^{\polylog (n)}$ many bits and we cannot afford to store all these bits during the execution of the algorithm $\A_n$. The subroutine $\S^*_n$ has the nice properties that (a) it has space complexity  $O(\poly (n))$ and (b) it can still  return the content of a given bit in $\mem_{\A^*}$ in $O(\polylog (n))$ time. In other words, the subroutine $\S^*_n$ stores the contents of $\mem_{\A^*}$ in an {\em implicit manner}, and whenever the subroutine $\A^*$ wants to read/write a given bit in $\mem_{\A^*}$, it does that by calling the subroutine $\S^*_n$. This ensures that the overall space complexity of $\A^*$ remains $O(\poly (n))$. However, the subroutine $\S^*_n$ will be able perform its designated task with $\polylog (n)$ update time and $\poly (n)$ space complexity only if the algorithm $\A_n$ is required to handle at most $\poly (n)$ many instance-updates after the preprocessing step. This is why we need~\ref{assume:poly:main} while defining the complexity classes $\dP$ and $\dNP$. 


\medskip
To summarize, we have shown that the algorithm $\A_n$  has polylog update time and polynomial space complexity. This implies that the $\fDNF$ problem is $\dNP$-hard. 











==> rankNP.tex <==

\section{The Class $\protect\drankNP$}

\label{sec:rankNP}

In this section, we define a class of dynamic problems called $\drankNP$
which we can later show its complete problems in \ref{sec:DNF}. The
class $\drankNP$ is contained in $\dNP$ yet still contains all known
problems in $\dNP$ to the best of our knowledge. 

The difference between $\dNP$ and $\drankNP$ is only that there
is an additional \emph{rank constraint }about a \emph{certifying proof-sequence}
(i.e. a proof-sequence that helps the verifier certifies each yes-instance).
More specifically, for $\drankNP$, there is a total order $\prec$
over all possible proof-updates which guarantees that if a proof-sequence
is inductively constructed according to $\prec$ at every step, then
such proof-sequence is a certifying proof-sequence. To contrast, for
$\dNP$, we only require that a certifying proof-sequence is inductively
constructed in arbitrary way.
\begin{defn}
[Class $\drankNP$]\label{def:rankNP}A decision problem $\D$ with
instance-update size $\lambda$ is in $\drankNP$ iff there is an
algorithm-family $\V$ such that, for any $n$, we have:
\begin{enumerate}
\item In the preprocessing step, $\V_{n}$ is given an initial instance
$I_{0}$ of size $n$. 
\item In each update step $t\ge1$, $\V_{n}$ is given an instance-update
$u(I_{t-1},I_{t})$ of size $\lambda(n)$ and a proof-update $\pi_{t}\in\{0,1\}^{\poly(\lambda(n))}$.
Then, $\V_{n}$ takes $\poly(\lambda(n))$ update time.
\end{enumerate}
Moreover, there is a total order $\prec_{\V_{n}}$ over $\{0,1\}^{\poly(\lambda(n))}$
such that, for any instance sequence $(I_{0},\dots,I_{k})$ of $\D$,
the following holds.\footnote{We stress that $\prec_{\V_{n}}$ does not depend on the instance sequence
$(I_{0},\dots,I_{k})$.} 
\begin{enumerate}
\item There is $(\pi_{1},\dots,\pi_{k})$ called the \emph{guaranteed proof-sequence}
(defined below) such that, for each $t$ where $\D(I_{t})=1$, then
$\V_{n}$ outputs $1$ at step $t$.
\item For any $(\pi_{1},\dots,\pi_{k})$ it holds that, for each $t$ where
$\D(I_{t})=0$, then $\V_{n}$ outputs $0$ or $\bot$ at step $t$.
\end{enumerate}
The guarantee proof sequence $(\pi_{1},\dots,\pi_{k})$ w.r.t. $(I_{0},\dots,I_{k})$
is inductively constructed as follows: for $t\ge1$, $\pi_{t}$ is
the first w.r.t. $\prec_{\V_{n}}$ such that $\V_{n}$ does not output
$\bot$ when $\V_{n}$ is given $(u(I_{t-1},I_{t}),\pi_{t})$ as input.
$\pi_{t}$ is called a \emph{guaranteed proof-update} at step $t$.

We say that $\V$ is a $\mbox{\ensuremath{\drankNP}}$-verifier-family
for $\D$. 
\end{defn}

\paragraph{Valid Outputs.}

When $\V_{n}$ outputs either $0$ or $1$, we say that \emph{$\V_{n}$
produces a valid output}, or equivalently the decision tree \emph{$T_{\V_{n}}$
produces a valid output}. Otherwise, $\V_{n}$ outputs $\bot$, then
we say $\V_{n}$ or $T_{\V_{n}}$ produces an \emph{invalid output}. 
\begin{prop}
$\dP\subseteq\drankNP\subseteq\dNP$.\end{prop}
\begin{proof}
Let $\A$ be a $\dP$-algorithm-family for a problem $\D$. Then,
$\A$ is also a $\drankNP$-verifier-family for $\D$ as $\A$ does
not even need to read the proofs. 

Let $\A'$ be a $\drankNP$-verifier-family for a problem $\D'$.
Then, $\A'$ is then an $\dNP$-verifier-family for $D'$. \ref{enu:NP yescase}
of \ref{def:NP} is implied by the existence of the guaranteed input
sequence. Next, \ref{enu:NP nocase} of \ref{def:NP} holds by slightly
modifying $\A'$ such that whenever the output is $\bot$, then output
$0$ instead. 
\end{proof}
We will see later that the restriction in the definition of $\drankNP$
can be exploited so that we can show complete problems for this class.
Below, we argue that this restriction is actually not so strict. In
particular, we do not know any problem which is in $\dNP$ but not
in $\drankNP$. 
\begin{thm}
All problems from \ref{table:BPP-NP} that are in $\dNP$ are actually
in $\drankNP$. (See \ref{sec:problem in rankNP} for the proofs.)
\end{thm}



==> related.tex <==
\section{Related Work}
\label{sec:related:work}

There are several previous attempts to classify dynamic problems.
First, there is a line of works called ``dynamic complexity theory''
(see e.g. \cite{DattaKMSZ15,WeberS05,SchwentickZ16}) where the general
question asks whether a dynamic problem is in the class called $\mbox{DynFO}$.
Roughly speaking, a problem is in $\mbox{DynFO}$ if it admits a dynamic
algorithm expressible by a first-order logic. This means, in particular, that given
an update, such algorithm runs in $O(1)$ parallel time, but might
take arbitrary $\mbox{poly}(n)$ works when the input size is $n$.
A notion of reduction is defined and complete problems of $\mbox{DynFO}$
and related classes are proven in \cite{HesseI02,WeberS05}.
However, as the total work of algorithms from this field can be large
(or even larger than computing from scratch using sequential algorithms), they do
not give fast dynamic algorithms in our sequential setting. 
Therefore, this setting is somewhat irrelevant to our setting.

Second, a problem called the \emph{circuit evaluation} problem has been shown to be
complete in the following sense. First, it is in $\mathsf{P}$ (the
class of static problems). Second, if the dynamic version of circuit
evaluation problem, which is defined as $\dDNF$ where a DNF-formula
is replaced with an arbitrary circuit, admits a dynamic algorithm
with polylogarithmic update time, then for any static problem $L\in\mathsf{P}$,
a dynamic version of $L$ also admits a dynamic algorithm with polylogarithmic
update time. This idea is first sketched informally since 1987 by
Reif \cite{Reif87}. Miltersen et al. \cite{MiltersenSVT94} then
formalized this idea and showed that other $\mathsf{P}$-complete
problems listed in \cite{miyano1990list,greenlaw1991compendium} also
are complete in the above sense\footnote{But they also show that this is not true for all $\mathsf{P}$-complete
	problems.}. The drawback about this completeness result is that the dynamic
circuit evaluation problem is extremely difficult. 
Similar to the case for static problems that reductions from $\mathsf{EXP}$-complete problems to problems in $\mathsf{NP}$ are unlikely, 
reductions from the dynamic circuit evaluation problem to other natural dynamic problems studied in the field seem unlikely. 
Hence, this does not give a framework for
proving hardness for other dynamic problems. 

Our result can be viewed as a more fine-grained completeness
result than the above. As we show that a very special case of the
dynamic circuit evaluation problem which is $\dDNF$ is already a
complete problem. An important point is that $\dDNF$ is simple enough
that reductions to other natural dynamic problems are possible. 

Finally, Ramalingam and Reps \cite{RamalingamR96} classify dynamic problems
according to some measure\footnote{They measure the complexity dynamic algorithms by comparing the update
	time with the size of \emph{change in input and output }instead of
	the size of input itself.}, but did not give any reduction and completeness result. 



==> test.tex <==

\section{Short proof: Hardness for the first DT problem}

Let $\V$ be the verifier for a problem $\D$. Let $\O$ be the oracle
for the \emph{first DT} problem $\D'$. We will show an algorithm
$\A$ with oracle $\O$ that can solve $\D$ with $\poly(\lambda_{\D}(n))$
update time when the initial instance is of size $n$ by describing
how $\A_{n}$ works for each $n$. 

Let $\T_{\V_{n}}$, $\prec_{\D_{n}}$ and $p(n)$ be defined as follows...

$\A_{n}$ will use $\V_{n}$ as a subroutine. 

At the preprocessing step (step 0), $\A_{n}$ works as follows:
\begin{enumerate}
\item $\A_{n}$ is given an initial input $\inp_{\A_{n}}(0)=I_{0}$, 
\item Let $\pi_{0}$ be the first proof according to $\prec_{\D_{n}}^{0}$
such that $\V_{n}((I_{0},\pi_{0}))\neq\bot$. 
\item Run $\V_{n}$ with an initial input $\inp_{\V_{n}}(0)=(I_{0},\pi_{0})$.
Let $\mem_{\V_{n}}(0)$ be the memory state of $\V_{n}$ at the end
of step $0$.
\item Set $I'_{0}=(\mem_{I'}(0),\prec_{I'},\ell_{I'},\T_{I'})=(\mem_{\V_{n}}(0),\prec_{\D_{n}},p(n),\T_{\V_{n}})$
as an initial input for the oracle $\O$.
\item Set the output at step 0 as $\A_{n}(\inp_{\A_{n}}(0))=\V_{n}(\inp_{\V_{n}}(0))$.
\end{enumerate}
At each update step (step $t\ge1$), we will keep the invariant that
$\mem_{I'}=\mem_{\V_{n}}$. $\A_{n}$ works as follows:
\begin{enumerate}
\item $\A_{n}$ is given an input $\inp_{\A_{n}}(t)=u(I_{t-1},I_{t})$ at
time $t$, 
\item We set $\mem_{\V_{n}}^{\inp}\gets u(I_{t-1},I_{t})$.
\item To keep the invariant, give a sequence of inputs to $\O$ that corresponds
to updating $\mem_{I'}=\mem_{\V_{n}}$. The length of the sequence
is at most $|u(I_{t-1},I_{t})|\le\lambda_{\D}(n)$.
\item Read the output $\pi_{t}$ from $\O$. We claim that $((I_{0}\pi_{0}),(u(I_{0},I_{1}),\pi_{1}),\dots,(u(I_{t-1},I_{t}),\pi_{t}))$
is a guaranteed sequence of input for $\V_{n}$.
\item Run $\V_{n}$ with an input $\inp_{\V_{n}}(t)=(u(I_{t-1},I_{t}),\pi_{t})$
at time $t$.
\item To keep the invariant, give a sequence of inputs to $\O$ that corresponds
to updating $\mem_{I'}=\mem_{\V_{n}}$. The length of the sequence
is at most $\poly(\lambda_{\D}(n))$ by the property of $\V_{n}$.
\item Set the output at step t as $\A_{n}(\inp_{\A_{n}}(0\rightarrow t))=\V_{n}(\inp_{\V_{n}}(0\rightarrow t))$.\end{enumerate}
\begin{lem}
For any $t\ge1$, $((I_{0}\pi_{0}^{*}),(u(I_{0},I_{1}),\pi_{1}^{*}),\dots,(u(I_{k-1},I_{k}),\pi_{k}^{*}))$
is a guaranteed sequence of input for $\V_{n}$.\end{lem}
\begin{proof}
By induction.\end{proof}
\begin{lem}
The update time of $\A_{n}$ with an oracle $\O$ is $\poly(\lambda_{\D}(n))$.\end{lem}
\begin{proof}
Clear.
\end{proof}

\section{Short proof: Easiness transferring}

Let $\R$ be a reduction from $\D$ to $\D'$. That is, $\R$ is an
algorithm with an oracle $\O$ for $\D'$ that can solve $\D$ with
$\poly(\lambda_{\D}(n))$ update time when the initial instance is
of size $n$. Let $\A'$ be a $\dP$-algorithm for $\D'$. We will
show a $\dP$-algorithm $\A$ for $\D$ by describing how $\A_{n}$
works for each $n$. 

$\A_{n}$ will use $\R_{n}$ and $\A'_{\qsize_{\R}(n)}$ as subroutines.

At the preprocessing step (step 0), $\A_{n}$ works as follows:
\begin{enumerate}
\item $\A_{n}$ is given an initial input $\inp_{\A_{n}}(0)=I_{0}$.
\item Run $\R_{n}$ with an initial input $\inp_{\R_{n}}(0)=I_{0}$. 
\item Let $I'_{0}$ be the string which $\R_{n}$ gives to the oracle $\O$
as an initial input. We have $|I'_{0}|=\qsize(n)$.
\item Run $\A'_{\qsize(n)}$ with an initial input $\inp_{\A'_{\qsize(n)}}(0)=I_{0}$.
\item Set the output at step 0 as $\A_{n}(\inp_{\A_{n}}(0))=\R_{n}(\inp_{\R_{n}}(0))$.
\end{enumerate}
At each update step (step $t\ge1$), $\A_{n}$ works as follows:
\begin{enumerate}
\item $\A_{n}$ is given an input $\inp_{\A_{n}}(t)=u(I_{t-1},I_{t})$ at
time $t$.
\item Simulate $\R_{n}$ with an input $\inp_{\R_{n}}(t)=u(I_{t-1},I_{t})$
on each operation (e.g. read/write/oracle-query) one by one as follows:

\begin{enumerate}
\item Run each read/write operation by $\R_{n}$ normally.
\item If the operation of $\R_{n}$ is to query $\O$ with some input $\inp_{\O}$. 
\item Run $\A'_{\qsize(n)}$ by giving the same input $\inp_{\A'_{\qsize(n)}}=\inp_{\O}$.
\item Let $\outp_{\A'_{\qsize(n)}}$ be the output of $\A'_{\qsize(n)}$.
We claim that $\outp_{\A'_{\qsize(n)}}=\outp_{\O}$ where $\outp_{\O}$
is the output from $\O$ if $\O$ is queried with $\inp_{\O}$.
\end{enumerate}
\item Set the output at step t as $\A_{n}(\inp_{\A_{n}}(0\rightarrow t))=\R_{n}(\inp_{\R_{n}}(0\rightarrow t))$.\end{enumerate}


